Generalized PTR: User-Friendly Recipes for Data-Adaptive Algorithms with Differential Privacy

The ''Propose-Test-Release'' (PTR) framework is a classic recipe for designing differentially private (DP) algorithms that are data-adaptive, i.e. those that add less noise when the input dataset is nice. We extend PTR to a more general setting by privately testing data-dependent privacy losses rather than local sensitivity, hence making it applicable beyond the standard noise-adding mechanisms, e.g. to queries with unbounded or undefined sensitivity. We demonstrate the versatility of generalized PTR using private linear regression as a case study. Additionally, we apply our algorithm to solve an open problem from ''Private Aggregation of Teacher Ensembles (PATE)'' -- privately releasing the entire model with a delicate data-dependent analysis.

==> Casestudy.tex <==
\section{Case Studies}
\label{sec:case_studies}

==> Generalized PTR (1)/Casestudy.tex <==
\section{Case Studies}
\label{sec:case_studies}

==> Generalized PTR (1)/PTR_calibration.tex <==


%  \vspace{-2mm}
% \subsection{``Which $\phi$ to propose?'' --- Generalized PTR with privacy calibration}
%     \vspace{-2mm}
%The optimism of all data-dependent analyses is to add less noise while maintaining the same or even stronger privacy guarantee compared to its data-independent counterpart. However, PTR approaches require a reasonable guess of the proposed parameter (e.g., $\lambda$ in the linear regression example). Otherwise, it may easily output $\perp$ and be less practical. Noting our generalized PTR takes an extra parameter $\phi$, one may hope to try out various $\phi$ (e.g., different noisy levels in private mean estimation) and return the one with the best utility. 
%In this section,  we propose an improved version of the generalized PTR such that the algorithm takes a list of parameters as input, runs PTR with each of the parameters, and only returns the output with the best utility. We show that the privacy guarantee in $\epsilon$ is independent of the number of $\phi$ that we try.  


% The main limitation of generalized PTR is that one needs to ``propose'' a good guess of parameter $\phi$.  Take the example of $\phi$ being the noise level in a noise-adding mechanism. Choosing too small a $\phi$ will result in a useless output $\perp$, while choosing too large a $\phi$ will add more noise than necessary.

% In this section,  we propose an improved version of generalized PTR such that the algorithm takes a list of parameters as input, runs PTR with each of the parameters, and only returns the output with the best utility. We show that the privacy guarantee in $\epsilon$ is independent of the number of $\phi$ that we try.  

% Formally, let $\phi_1, ..., \phi_k$ be a set of hyper-parameters and $\tilde{\theta}_i \in\{\perp, \text{Range}(\cM)\}$ denotes the output of running generalized PTR on a private dataset $X$ with $\phi_i$. 
% Let $X_{val}$ be a public validation set and $q(\tilde{\theta}_i)$ be the score of evaluating $\tilde{\theta}_i$ with $X_{val}$ (e.g., validation accuracy). The goal is to select a pair of DP model $\tilde{\theta}_i$ and its  hyper-parameter $\phi_i$, such that $\tilde{\theta}_i$ maximizes the validation score.

%(1) the system is $(\tilde{\epsilon}, \tilde{\delta})$-DP; (2) the validation score $q(\theta_i) \geq max_j q(\theta_j) -\alpha$ with high probability.


%The generalized PTR with privacy calibration is described in Algorithm~\ref{alg: parameter_ptr}. Specifically, $T$ denotes the computational limit. We assume an oracle access to the score function $(\tilde{\theta}_i, q(\tilde{\theta}_i)) \sim Q(X)$ by: (a) pick a candidate $\phi_i$ randomly; If there is an order between parameters (e.g., $\phi_i$ denotes the magnitude of noise level), then we can sort $\phi_i$ such that $\phi_1 < \phi_2 < ... < \phi_k$ and pick $\phi_i$ from the left; (b) Run
%Algorithm~\ref{alg:gen_ptr} to obtain $\tilde{\theta}_i$ and evaluate it on $X_{\text{val}}$. Finally, the algorithm outputs the highest scored candidates.


% Finally, the algorithm has a random stopping with probability $\gamma$. 
% state privacy guarantee, cite from 
% The generalized PTR framework with privacy calibration is described in Algorithm~\ref{alg: parameter_ptr}. The privacy guarantee of Algorithm~\ref{alg: parameter_ptr} is an application of \citet{liu2019private}.

% \begin{theorem}[ Theorem 3.4 \citet{liu2019private} ]
% Fix any $\tau \in [0, 1], \delta_2>0$ and let $T =\frac{1}{\tau} \log \frac{1}{\delta_2}$. If each oracle access to $Q(X)$ is $(\epsilon, \delta)$-DP, then
% Algorithm~\ref{alg: parameter_ptr} is $(3\epsilon + 3\sqrt{2\delta}, \sqrt{2\delta} T +\delta_2 )$-DP.%\yw{What if it does not reach $T$? Also in the algorithm it has $k$ right?  Also, did you define which score it is?}
% \end{theorem}
% The theorem implies that one can try a random number of $\phi$ while paying a constant $\epsilon$.
% In practice, we can roughly set $\tau = \frac{1}{10k}$ so that the algorithm is likely to test all $k$ parameters. We emphasize that the privacy and the utility guarantee (see Sec~\ref{sec: omit_gen_ptr} in Appendix) is not our contribution. But the idea of applying a generalized PTR to enforce a uniform DP guarantee over all choices of parameters with data-dependent analysis is new, and in our opinion, significantly broadens the applicability to generic hyperparameter tuning machinery from \citep{liu2019private}.




%\begin{remark}[Private hyper-parameter tuning]
%Our results directly generalize private hyper-parameter tuning. We remark that our PTR-based algorithm can tune privacy parameters (e.g., noise scale) adapted to the data-dependent DP while maximizing the utility. In contrast, prior work~\citep{papernot2021hyperparameter}\citep{liu2019private} on this problem requires a uniform DP guarantee of all base mechanisms, thus not applicable. 
%\end{remark}


%We can categorize hyper-parameters of privacy-preserving models into two sets --- utility parameters and privacy parameters. 

%Most prior work~\citep{liu2019private, papernot2021hyperparameter} on this problem assumes parameters of interests are privacy uncorrelated (e.g., regularizer parameter) and require a uniform DP bound for all of the mechanisms $\cM_i$.  \citet{liu2019private} shows that if each mechanism $\cM_i$ is $(\epsilon, 0)$-DP, then run a random number of mechanisms and report the best option satisfies $(3\epsilon, 0)$-DP.

 %On the other hand, for noise calibration with a fixed privacy budget, we note that one could naively apply a differential privacy accountant (e.g., Renyi DP accountant \citep{mironov2017renyi}) to apriori optimize the privacy parameters with a fixed privacy budget. However, this approach does not give us insights into the utility guarantee or take advantage of the data-dependent property. 

%We generalize the above results by: (1) considering a wide range of hyper-parameters that could be either privacy parameters or non-privacy parameters. (2) Tune parameters adapted to the dataset itself.

%\yw{The two paragraphs above are not clear (from ``on the other hand'' onwards). Should  revise so readers understand what you mean.} % i have remove it to the related work.


% \begin{algorithm}[t]
% 	\caption{PTR with hyper-parameter selection}
% 	\label{alg: parameter_ptr}
% 	\begin{algorithmic}[1]
% 	   \STATE {\textbf{Input}:  Privacy budget $\epsilon, \delta$, cut-off $T$, parameters $\phi_{1:k}$, flipping probability $\tau$ and the access to the validation score $q(\cdot)$. } 
% 		\STATE {Initialize the set $S=\varnothing$.}
% 		\STATE{Draw $G$ from a geometric distribution $\cD_\tau$ and let $\hat{T}=\text{min}(T, G)$.}
% 		\FOR{i = 1 ,..., $\hat{T}$}
% 		\STATE{ pick a random $\phi_i$ from $\phi_{1:k}$.}
% 		\STATE{evaluate $\phi_i$: $(\tilde{\theta}_i, q(\tilde{\theta}_i))\gets$ Algorithm~\ref{alg:gen_ptr}($\phi_i, (\epsilon, \delta)$).}
% 		\STATE {$S \gets S \cup \{\tilde{\theta}_i, q(\tilde{\theta}_i)\}$.}
% 		%\STATE{with probability $\gamma$, we output the highest scored candidate from $S$ and halt.}
% 		\ENDFOR	\vspace{-1mm}
% 	\STATE{Output the highest scored candidate from $S$.}
% 	\end{algorithmic}
% 	\vspace{-1mm}
% \end{algorithm}

% \begin{figure*}[t]
% 	\centering	
% 	\subfigure[Bike dataset]{
% 	\includegraphics[width=0.48\textwidth]{img/bike.pdf}\label{fig:bike}}
% 	\subfigure[Elevators dataset]{
% 	\includegraphics[width=0.48\textwidth]{img/elevator.pdf}\label{fig:ele}}
% 	\vspace{-2mm}
% 	\caption{Differential private linear regression algorithms on UCI datasets. $y$-axis reports the MSE error with confidence intervals. $\epsilon$ is evaluated with $\delta = 1e-6$. }
% 	\label{fig:selection}\vspace{-2mm}
% \end{figure*}

\textbf{Case study with private linear regression.}
We next apply Algorithm~\ref{alg: parameter_ptr} to the private linear regression task with UCI regression datasets. Standard z-scoring is applied and each data point is normalize with a Euclidean norm of 1.  We consider $(60\%,10\%,30\%)$ splits for training, validation and testing test.

\textbf{Baselines}
\begin{itemize}
\vspace{-2mm}
    \item Output Perturbation (Outpert)~\citep{chaudhuri2011differentially}: $\theta=(X^TX + \lambda I)^{-1}X^T\bf{y}$. Release $\hat{\theta} = \theta + \bf{b}$ with an appropriate $\lambda$ and $\bf{b}$ is a Gaussian random vector.\vspace{-2mm}
    \item Posterior sampling (OPS). Sample $\hat{\theta}\sim P(\theta)\propto e^{-\gamma(F(\theta)+ 0.5 \lambda ||\theta||^2)}$ with parameters $\gamma, \lambda$.\vspace{-1.5mm}
    \item Adaptive posterior sampling (AdaOPS)~\citep{wang2018revisiting}. Run OPS with $(\lambda, \gamma)$ chosen adapted to the dataset.\vspace{-1.5mm}
\end{itemize}
%\yw{\cite{gopi2022private} had a nice and clean Gaussian DP bound for OPS. I thought if we can privately test the strong convexity from the dataset, it should satisfy a stronger Gaussian DP. How are privacy accounted in the experiments now?} % use composition.  Each oracle call is (eps, delta). split (epsilon/2, delta/2) to release data dependent quantity, use the remaining to tune gamma for an input lambda.
Outpert and OPS serve as two non-adaptive baselines. In particular, we consider OPS-Balanced~\citep{wang2018revisiting}, which chooses $\lambda$ to minimize a data-independent upper bound of empirical risk and dominates other OPS variants. 
AdaOPS is one state-of-the-art algorithm for adaptive private regression, which  automatically chooses $\lambda$ by minimizing an upper bound of data-dependent empirical risk.


We implement OPS-PTR as follows: 
propose a list of $\lambda$ through grid search (we choose $k=30$ and $\lambda$ ranges from $[2.5, 2.5^{10}]$ on a logarithmic scale); instantiate Algorithm~\ref{alg: parameter_ptr} with $\tau =0.1k, T=\frac{1}{\tau} \log(1/\delta_2)$ and  $\delta_2 = 1/2 \delta$;
calibrate $\gamma$ to meet the privacy requirement for each $\lambda$. sample $\hat{\theta}$ using $(\lambda,\gamma)$ and return the one with the best validation accuracy. Notice that we use a ``no $\perp$'' variant of Algorithm~\ref{alg:gen_ptr} as the calibration of $\gamma$ is clear given a fixed $\lambda$ and privacy budget (see more details in the appendix). We can propose various combinations of $(\lambda, \gamma)$ for more general applications.


 Figure~\ref{fig:selection}  demonstrates how  the MSE error of the linear regression algorithms vary with the privacy budget $\epsilon$. OutPert suffers from the large global sensitivity of output $\theta$. OPS performs well but does not benefit from the data-dependent quantities. Alternatively, AdaOPS is able to choose $(\lambda, \gamma)$ adapted to the dataset, but suffers from the estimation error of the data-dependent empirical risk. On the other hand, OPS-PTR chooses a  $(\lambda, \gamma)$ pair that minimizes the empirical error on the validation set directly, and the privacy parameter $\gamma$ is adapted to the dataset thus achieving the best result.




==> Generalized PTR (1)/applications.tex <==
\section{Applications}
% \vspace{-1.em}
\label{sections:applications}
In this section, we put into action our approaches to construct the DP test and provide applications in private linear regression and PATE.





%  \vspace{-2mm}
% \subsection{``Which $\phi$ to propose?'' --- Generalized PTR with privacy calibration}
%     \vspace{-2mm}






\subsection{Private Linear Regression}

\input{private_linear_regression}
\label{subsections:private_linear_regression}




\subsection{PATE}
\label{subsections:pate}
\input{pate}


==> Generalized PTR (1)/conclusion.tex <==
\section{Limitations and Future Work}
One weakness of generalized PTR is that it requires a case-specific privacy analysis. Have we simply exchanged the problem of designing a data-adaptive DP algorithm with the problem of analyzing the data-dependent privacy loss? We argue that this limitation is inherited from classic PTR. In situations where classic PTR is not applicable, we've outlined several approaches to constructing the DP test for our framework (see Sections~\ref{subsections:test_construction} and~\ref{section:applications}).

Furthermore, the data-dependent privacy loss is often more straightforward to compute than local sensitivity, and often exists in intermediate steps of classic DP analysis already. Most DP analysis involves providing a high-probability tail bound of the privacy loss random variable. If we stop before taking the max over the input dataset, then we get a data-dependent DP loss right away (as in Example~\ref{examp:lap_mech}).

There are several exciting directions for applying generalized PTR to more problems. Sufficient statistics release and our private hyperparameter tuning (Algorithm~\ref{alg: parameter_ptr}) can be used to construct data-adaptive extensions of DP-PCA \citep{dwork2014analyze} and Sparse-DP-ERM \citep{kifer2012private}. For DP-PCA we could use our Algorithm~\ref{alg: parameter_ptr} to tune the variance of the noise added to the spectral gap; for Sparse-DP-ERM we would test the restricted strong convexity parameter (RSC), i.e. not adding additional regularization if the RSC is already large.


\section{Conclusion}

Generalized PTR extends the classic ``Propose-Test-Release'' framework to a more general setting by testing the data-dependent privacy loss of an input dataset, rather than its local sensitivity. In this paper we've provided several examples -- private linear regression with hyperparameter selection and PATE -- to illustrate how generalized PTR can enhance DP algorithm design via a data-adaptive approach.

==> Generalized PTR (1)/expost.tex <==

\subsection{Ex-post DP}

\begin{theorem}
Algorithm~\ref{alg: ptr_gen_post} is $(\max(\epsilon_1 +\epsilon_2, \epsilon_2 -\epsilon_1 +\nu), 2\delta_2 +e^{\epsilon_2}\cdot \delta)$-DP if with probability at least $1-\delta$, we have $\epsilon(\theta, X)\leq \epsilon_\phi(X, \theta)^p\leq \epsilon_\phi(X,\theta) + \nu$ for any neighboring dataset $X'$.
\end{theorem}

\begin{proof}

Let $\tilde{\cM}$ denote Algorithm~\ref{alg: ptr_gen_post}.
We consider two cases: $\tilde{\cM}(X)=\perp$ and $\tilde{\cM}(X)=\theta$.
The probability of outputting $\perp$ can be written explicitly as follows:
\begin{align*}
&\pr[\tilde{\cM}(X)=\perp] = \pr_{\tilde{\cM}(X)}[\epsilon(\theta, X)^p>\epsilon_1]\\
&= \mathbb{E}_{\theta \sim \cM(X)}\bigg[ \pr_{\cA(X, \theta)}[\epsilon(\theta, X)^p >\epsilon_1|\theta]\bigg]\\
&\leq e^{\epsilon_2} \underbrace{{\mathbb{E}_{\theta \sim \cM(X)}\bigg[ \pr_{\cA(X',\theta)}\bigg[\epsilon(\theta, X')^p >\epsilon_1|\theta\bigg]\bigg]}}_{\text{denoted by} (*) } + \delta_2\\
\end{align*}
The inequality in the last line uses the definition of DP of $\cA(X,\theta)$, which satisfies $(\epsilon_2, \delta_2)$-DP.
Then our goal is to bound $(*)$.  Using the assumption ``w.h.p. $1-\delta$, $\epsilon(\theta, X)\leq \epsilon(X, \theta)^p\leq \epsilon(X,\theta) + \nu$, we have 

\[ (*)\leq \mathbb{E}_{\theta \sim \cM(X)}\bigg[ \pr_{\cA(X',\theta)}\bigg[\epsilon(\theta, X')^p >\epsilon_1
\cap E | \theta \bigg]\bigg] + \delta\]
where $E$ denotes the event of $\epsilon(\theta, X)\leq \epsilon(X, \theta)^p\leq \epsilon(X,\theta) + \nu$.

Note that \[\epsilon(\theta, X')^p \leq \epsilon(\theta, X') +\nu = \log \frac{\pr_{\cM(X')}(\theta)}{\pr_{\cM(X)}(\theta)} + \nu\], which combines with $\epsilon(\theta,X')^p>\epsilon_1$, gives us $\log \frac{\pr_{\cM(X)}(\theta)}{\pr_{\cM(X')}(\theta)} \leq -\epsilon_1 + \nu$. This inequality further implies $\pr_{\cM(X)}(\theta)\leq e^{\nu-\epsilon_1}\cdot \pr_{\cM(X')}(\theta)$.

Substituting the above expression to $(*)$ and we obtain
\begin{align*}
&(*) \leq e^{\nu -\epsilon_1}\cdot \mathbb{E}_{\theta \sim \cM(X')} \bigg[\pr_{\cA(X', \theta)}\bigg[\epsilon(X', \theta)^p >\epsilon \cap E \bigg]\bigg] + \delta\\
&\leq e^{-\epsilon_1 + \nu}\cdot \pr[{\tilde{\cM}(X')=\perp}] + \delta
\end{align*}
Therefore, we have 
\begin{align*}
& \pr[\tilde{\cM}(X)=\perp] \leq e^{\epsilon_2}\bigg(e^{-\epsilon_1 +\nu}\cdot \pr[\tilde{\cM}(X')=\perp ]+\delta\bigg)+ \delta_2\\
&= e^{\epsilon_2 -\epsilon_1 +\nu}\cdot \pr[\tilde{\cM}(X')=\perp] + \delta\cdot \epsilon^{\epsilon_2} +\delta_2
\end{align*}
We next proceed to bound the other case --- $\pr[\tilde{\cM}(X) \in S]$, where $S \subset Range(\cM)$.

 The probability of outputting $S \subset Range(\cM)$ is as follows:
 \begin{align}
 & \pr[\tilde{\cM}(X)\in S)] \\
 &= \underbrace{\mathbb{E}_{\theta \sim \cM(X)}\bigg[ \pr_{\cA(X,\theta)}\bigg[  \epsilon(X, \theta)^p\leq \epsilon_1, E|\theta \bigg]\mathbb{1}(\theta\in S)\bigg]}_{\text{denoted by} (*)} + \\
 & \underbrace{\mathbb{E}_{\theta \sim \cM(X)}\bigg[ \pr_{\cA(X,\theta)}\bigg[  \epsilon(X, \theta)^p\leq \epsilon_1, E^c |\theta\bigg] \mathbb{1}(\theta\in S)\bigg]}_{\text{denoted by} (**)}
\end{align}, where $E$ denotes the event of $\epsilon(\theta, X)\leq \epsilon( \theta,X) +\nu$.
Similarly, we apply the post-processing property on $(*)$ and we have
\begin{align}
&(*)\leq \mathbb{E}_{\theta \sim \cM(X)}\bigg[\bigg( \pr_{\cA(X',\theta)}[\epsilon(\theta, X')\leq \epsilon(\theta, X')^p\leq \epsilon_1|\theta]\cdot \epsilon^{\epsilon_2}+\delta\bigg)
\mathbb{1}(\theta \in S)\bigg]\\
&\leq e^{\epsilon_2}\int_S \pr[\cM(X)=\theta]\pr_{\cA(\theta, X')}[\epsilon(\theta, X')\leq \epsilon(\theta, X')^p \leq \epsilon_1]d\theta + \delta_2\\
&=e^{\epsilon_2}\int_S \int_{\epsilon(\theta, X')}^{\epsilon_1} \pr[\cM(X)=\theta]\pr_{\cA(\theta, X')}[\epsilon(\theta, X')^p]d \epsilon(\theta, X')^p d\theta + \delta \label{ine: change}\\
&\leq e^{\epsilon_2}\int_S \int_{\epsilon(\theta, X')}^{\epsilon_1}e^{\epsilon_1} \pr[\cM(X')=\theta] \pr_{\cA(\theta, X')}
\epsilon(\theta, X')^p d\epsilon(\theta, X')^pd\theta +\delta_2\\
&=e^{\epsilon_1 +\epsilon_2}\mathbb{E}_{\theta\sim \cM(X')}\bigg[ \pr_{\cA(\theta, X')}[\epsilon(\theta,X')\leq \epsilon(\theta, X')^p \leq \epsilon_1|\theta]\cdot \mathbb{1}(\theta \in S)\bigg] + \delta_2\\
&\leq e^{\epsilon_1 + \epsilon_2} \pr_{\theta \sim \cM(X')}[\theta \in S]+\delta_2
\end{align}
In Inequality~\ref{ine: change}, $\epsilon(\theta, X')^p \leq \epsilon_1 $ implies $\pr(\cM(X)=\theta)\leq e^{\epsilon_1}\cdot \pr[\cM(X')=\theta]$, which allows us to replace $\cM(X)=\theta$ with $\cM(X')=\theta$ in the next step.
For $(**)$, given that $\pr_{\cA(\theta, X)}[\epsilon(\theta, X)>\epsilon(\theta,X')^p]\leq \delta$, we have $(**)\leq \delta$. Therefore, we have 
\[\pr[\tilde{\cM}(X)\in S] \leq e^{\epsilon_1 + \epsilon_2 } \pr[\tilde{\cM}(X')\in S] + \delta_2 + \delta
\]
Combine the case of $\tilde{\cM}(X)=\perp$ and $\tilde{\cM}(X)\in \{Range(\cM)\}$, we have $\forall \tilde{S} \subset \{ Range(\cM) \cup \{\perp\}\}$:
\begin{align*}
    &\pr[\tilde{\cM}(X)\in \tilde{S}] = \pr[\tilde{\cM}(X) \in \tilde{S} \cap \perp^c] + \pr[\tilde{\cM}(X) = \perp]\\
    &\leq e^{\epsilon_1 + \epsilon_2}\pr[\tilde{\cM}(X) \in \tilde{S} \cap \perp^c] + e^{\epsilon_2 -\epsilon_1 +\nu}\pr[\tilde{\cM}(X')=\perp] + 2\delta_2 + e^{\epsilon_2} \delta
\end{align*}
\end{proof}

==> Generalized PTR (1)/genPTR.tex <==
%\vspace{-1em}
\section{Generalized PTR}
%\vspace{-1em}
\label{sec:gen_ptr}
This section introduces the generalized PTR framework. We first formalize the notion of \emph{data-dependent} differential privacy that conditions on an input dataset $X$. 

\begin{definition}[Data-dependent privacy]
\label{def:data_dep_dp}
Suppose we have $\delta > 0$ and a function $\epsilon: \mathcal{X} \rightarrow \mathbb{R}$. We say that mechanism $\mathcal{M}$ satisfies ($\epsilon(X), \delta$) data-dependent DP\footnote{We will sometimes write that $\cM(X)$ satisfies $\epsilon(X)$ data-dependent DP with respect to $\delta$.} for dataset $X$ if for all possible output sets $S$ and neighboring datasets $X'$,
\begin{align*}
    \text{Pr}\big[\mathcal{M}(X) \in S\big] &\leq e^{\epsilon(X)}\text{Pr}\big[\mathcal{M}(X') \in S\big] + \delta, \\
       \text{Pr}\big[\mathcal{M}(X') \in S\big] &\leq e^{\epsilon(X)}\text{Pr}\big[\mathcal{M}(X) \in S\big] + \delta.
\end{align*}
\end{definition}

In generalized PTR, we propose a value $\phi$ for the randomized algorithm $\cM$, which could be a noise scale or regularization parameter -- or a set including both. For example, $\phi = (\lambda, \gamma)$ in Example~\ref{exp: posterior}. We then say that $\cM_{\phi}$ is the mechanism $\mathcal{M}$ parameterized by $\phi$, and $\epsilon_{\phi}(X)$ its data-dependent DP.

The following example illustrates how to derive the data-dependent DP for a familiar friend -- the Laplace mechanism.

\begin{example}(\emph{Data-dependent DP of Laplace Mechanism.}) \label{examp:lap_mech}
Given a function $f: \mathcal{X} \rightarrow \mathbb{R}$, we will define
\begin{align*}
    \mathcal{M}_{\phi}(X) = f(X) + \text{Lap}\left(\phi\right).
\end{align*}
We then have
\begin{align*}
    \log \dfrac{\emph{Pr}[\mathcal{M}_{\phi}(X) = y]}{\emph{Pr}[\mathcal{M}_{\phi}(X') = y]} &\leq \dfrac{|f(X) - f(X')|}{\phi}.
\end{align*}
Maximizing the above calculation over all possible outputs $y$ and using Definition~\ref{def:data_dep_dp},
\begin{align*}
    \epsilon_{\phi}(X) = \max\limits_{X': X' \simeq X} \frac{|f(X) - f(X')|}{\phi} = \frac{\Delta_{LS}(X)}{\phi}.
\end{align*}
% We can then verify that choosing $\phi = \beta/\hat{\epsilon}$ and $\hat{\epsilon} = \epsilon$ reduces Algorithm~\ref{alg:no_ls} exactly to Algorithm~\ref{alg:classic_ptr}.
\end{example}


The data-dependent DP $\epsilon_\phi(X)$ is a function of both the dataset $X$ and the parameter $\phi$. Maximizing $\epsilon_\phi(X)$ over $X$ recovers the standard DP guarantee of running $\cM$ with parameter $\phi$.


 %We take the functional view of $\epsilon_\phi(X)$ and use $\epsilon_{\phi, \delta}(X)$ to denote the $\epsilon$ as a function of $\delta$.
  % Add what is data-dependent dp, it's a function representation

 
%  Suppose we are given an $(\epsilon, \delta)$-DP test $\mathcal{T}$ that fails with probability $\Tilde{\delta}$ in order to determine whether or not $\mathcal{M}_{\phi}$ satisfies ($\hat{\epsilon}, \hat{\delta}$)-DP. Based on the outcome of $\mathcal{T}$,  we decide whether to run $\mathcal{M}_{\phi}$ or to halt and return $\perp$.
 
\begin{figure}[H]
%\vspace{-1em}
\centering
% \resizebox{0.95\columnwidth}{!}{%
% \begin{minipage}{0.54\textwidth}
\begin{algorithm}[H]
\caption{Generalized Propose-Test-Release}
\label{alg:gen_ptr}
\begin{algorithmic}[1]
\STATE{\textbf{Input}: Dataset $X$; mechanism $\cM_\phi: \mathcal{X} \rightarrow \cR$ and its privacy budget $\epsilon, \delta$; $(\hat{\epsilon}, \hat{\delta})$-DP test $\mathcal{T}$; false positive rate $\leq \delta'$; data-dependent DP function $\epsilon_\phi(\cdot)$ w.r.t. $\delta$}.
% \STATE{\blue{Run a test $\mathcal{T}$ to determine if $\cM_\phi$ is $(\hat{\epsilon}, \hat{\delta})$-DP at $X$.}}
% \STATE{\textbf{if} the test $\mathcal{T}$ passes \textbf{then} release $\theta = \mathcal{M}_{\phi}(X)$.}\vspace{-1pt}
\STATE{\textbf{if not} $\mathcal{T}(\cX)$ \textbf{then} output $\perp$,}\vspace{-1pt}
\STATE{\textbf{else} release $\theta = \mathcal{M}_{\phi}(X).$}%\vspace{-2pt}
\end{algorithmic}
\end{algorithm}
\end{figure}

 
\begin{theorem}[Privacy guarantee of generalized PTR]
\label{thm:gen_ptr}
Consider a proposal $\phi$ and a data-dependent DP function $\epsilon_{\phi}(X)$ w.r.t. $\delta$. Suppose that we have an ($\hat{\epsilon}, \hat{\delta}$)-DP test $\cT: \cX \rightarrow \{0, 1\}$ such that when $\epsilon_{\phi}(X) > \epsilon$, \end{theorem}
\vspace{-8mm}
\begin{align*}
    \cT(X) =
    \begin{cases}
        0  \text{ \:with probability } 1 - \delta', \\
        1  \text{\: with probability }  \delta'. %\vspace{-2mm}
    \end{cases}
\end{align*}
%\vspace{-2mm}
\textit{Then Algorithm~\ref{alg:gen_ptr} satisfies ($\epsilon + \hat{\epsilon}, \delta +  \hat{\delta} + \delta'$)-DP. }
% \vspace{-2mm}
%  \end{theorem}
 \begin{proof}[Proof sketch]
 There are three main cases to consider:
\begin{enumerate}
    %\vspace{-1em}
    \item We decide not to run $\mathcal{M}_{\phi}$.   % \vspace{-0.5em}
    \item We decide to run $\mathcal{M}_{\phi}$ and $\epsilon_{\phi}(X) > \epsilon$;    %\vspace{-0.5em}
    \item We decide to run $\mathcal{M}_{\phi}$ and $\epsilon_{\phi}(X) \leq \epsilon$.    %\vspace{-0.5em}
\end{enumerate}%\vspace{-2mm}
In the first case, the decision to output $\perp$ is post-processing of an $(\hat{\epsilon}, \hat{\delta})$-DP mechanism and inherits its privacy guarantees. The second case occurs when the $(\hat{\epsilon}, \hat{\delta})$-DP test "fails" (produces a false positive) and occurs with probability at most $\delta'$. The third case is a composition of an $(\hat{\epsilon}, \hat{\delta})$-DP algorithm and an ($\epsilon, \delta$)-DP algorithm.
 \end{proof}
 
% The construction of the test required by Theorem~\ref{thm: gen_ptr}
% can be flexibly adapted to any use case. We outline two  approaches to construct such a test in Sec~\ref{section:applications}. 

% \blue{Theorem~\ref{thm: gen_ptr} requires a private test $\mathcal{T}$ to be clear.   The data-dependent privacy loss might depend on the dataset in different ways, and thus the derivation of the test requires a case-specific study. We outline two approaches to construct such a test in Sec~\ref{section:applications}. }
% Before we reach that point, we first show that the classic PTR (Algorithm~\ref{alg:classic_ptr}) can be viewed under our framework as Algorithm~\ref{alg:gen_ptr} instantiated with a specific type of test.
% \begin{theorem}[Generalized PTR with distance test]\label{exp: dist_ptr}
% Let $\delta, \delta' > 0$ and define an algorithm $\cA: \cR^d \to \{\perp, \cR^d\}$ as follows.
% Let $\gamma(X)$ denote the distance to the nearest dataset $X''$ such that $\epsilon_{\phi, \hat{\delta}}(X'')>\hat{\epsilon}$, i.e.,
% $\gamma(X) = \min_{X''} \{dist(X, X''):\epsilon_{\phi, \hat{\delta}}(X'')>\hat{\epsilon}\}$. Let $\mathcal{T}$ test whether $ \gamma(X)+ Lap(1/\epsilon)>\frac{\log(1/\tilde{\delta})}{\epsilon}$.
%   $\cA$ returns $\cM_\phi(X)$ if $\mathcal{T}$ passes and otherwise returns $\perp$. Then $\cA$ is $(\epsilon+\hat{\epsilon}, \hat{\delta}+ \tilde{\delta})$-DP. 
% \end{theorem}
% \blue{Look at this again! Are the deltas correct?}



Generalized PTR is a \emph{strict} generalization of Propose-Test-Release. For some function $f$, define  $\cM_{\phi}$ and $\cT$ as follows:
\begin{align*}
&\mathcal{M}_{\phi}(X) = f(X) + \text{Lap}(\phi); \\
&\cT(X) = 
\begin{cases}
0 & \text{ if\:\: } \cD_{\beta}(X) + \text{Lap}\left(\frac{1}{\epsilon}\right) > \frac{\log(1/\delta)}{\epsilon},\\
1 & \text{ otherwise.} \\
\end{cases}
\end{align*}
Notice that our choice of parameterization is $\phi = \frac{\beta}{\epsilon}$, where $\phi$ is the scale of the Laplace noise. In other words, we know from Example~\ref{examp:lap_mech} that $\epsilon_{\phi}(X) > \epsilon$ exactly when $\Delta_{LS}(X) > \beta$.

For noise-adding mechanisms such as the Laplace mechanism, the sensitivity is proportional to the privacy loss (in both the global and local sense, i.e. $\Delta_{GS} \propto \epsilon$ and $\Delta_{LS} \propto \epsilon(X)$). Therefore for these mechanisms the only difference between privately testing the local sensitivity (Algorithm~\ref{alg:classic_ptr}) and privately testing the data-dependent DP (Theorem~\ref{thm:gen_ptr}) is a change of parameterization.
%\vspace{-0.5em}
\subsection{Limitations of local sensitivity}
%\vspace{-1em}
\input{local_sensitivity_examples}
\label{subsections:local_sensitivity}
%\vspace{-1em}
\subsection{Which $\phi$ to propose}
%\vspace{-0.5em}
% upper bound apporach and hyperparameter tuning
\input{which_phi}
\label{subsections:which_phi}

\input{hyperparameter_selection}
%\vspace{-0.5em}
\subsection{Construction of the DP test}
\input{test_construction}
\label{subsections:test_construction}

%  Next, we provide another instantiation of generalized PTR through the construction of a high-probability upper bound of $\epsilon_{\phi}(X)$.








% \blue{Compared to  classic PTR, the key idea of the procedure above is that we can construct a ``sanitized'' upper bound of $\epsilon_\phi(X)$ instead of local sensitivity, which always exists.  Moreover, the above framework allows us to be more flexible in both the type of test conducted and also the type of mechanism whose output we wish to release.}
% \blue{Put the above into the 'Unified Framework section?'}


%In particular, our result suggests that one can privately publish any mechanism $\cM$ with a data-dependfent analysis through publishing $\epsilon_\phi(X)$, which captures sufficient statistics of the dataset, and is less costly as it is a real-valued number rather than a $d$-dimensional model $\cM$.
% \begin{figure}[t]
% \vspace{-1em}
% \centering
% \resizebox{0.95\columnwidth}{!}{%
% \begin{minipage}{0.54\textwidth}
% \begin{algorithm}[H]
% \caption{Propose-Test-Release \cite{dwork2009differential}}
% \label{alg:classic_ptr}
% \begin{algorithmic}[1]
% \STATE{\textbf{Input}: Dataset $X$; privacy parameters $\epsilon,\delta$; proposed bound $\beta$ on $\Delta_{LS}(X)$; query function $f: \mathcal{X} \rightarrow \mathbb{R}$.}
% \STATE{\textbf{Output}: $f^P(X)$ or $\perp$.}
% \STATE{Compute the distance $\gamma(X)$ to the nearest dataset $X''$ such that $ \Delta_{LS}(X'')> \beta$:
% $\gamma(X) = \min\limits_{X''} \{ \text{dist}(X, X''): \Delta_{LS}(X'')> \beta \}$.}
% \STATE{Privately release $\gamma^P(X) = \gamma(X) + \text{Lap}\left(\frac{1}{\epsilon}\right)$.}
% \STATE{\textbf{if} $\gamma^P(X) \leq \dfrac{\log(1/\delta)}{\epsilon}$ \textbf{then} output $\perp$}\vspace{-1pt}
% \STATE{\textbf{else} release $f^P(X) = f(X) + \text{Lap}\left(\frac{\beta}{\epsilon}\right)$.}\vspace{-2pt}
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \quad
% \begin{minipage}{0.45\textwidth}
% \begin{algorithm}[H]
% \caption{Generalized PTR}
% \label{alg:gen_ptr}
% \begin{algorithmic}[1]
% \STATE{{Input}: Proposed~parameter~$\phi$;~privacy~parameters~$\epsilon,  \hat{\epsilon}, \hat{\delta}$; dataset $X$;\blue{an -$(\epsilon,\delta)$~DP test $\cT$ with false positive rate at most $\tilde{\delta}$; ~data-dependent~DP~function~$\epsilon_{\phi}(\cdot, \hat{\delta})$;~mechanism~$\mathcal{M}_{\phi}$.}}
% \STATE{\textbf{Output}: 
% $\mathcal{M}_{\phi}(X)$ or $\perp$.}
% \STATE{\blue{Run a test $\cT$ to determine if $\cM_{\phi}$ is $(\hat{\epsilon}, \hat{\delta})$-DP at $X$.}}% with privacy limit $(\hat{\epsilon}, \hat{\delta})$ }.
% \IF{the test $\cT$ passes}
% \vspace{1pt}
% \STATE{Run $\theta = \mathcal{M}_{\phi}(X)$ and output $\theta$.}%\vspace{2pt}
% \ELSE 
% \STATE{Output $\perp$.}%\vspace{2pt}

% \ENDIF
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% }
% \vspace{-1em}
% \end{figure}







% \begin{comment}
% \begin{example}(\emph{Laplace Mechanism}) \label{examp:lap_mech}

% Given a function $f: \mathcal{X} \rightarrow \mathbb{R}$, we will define
% \begin{align*}
%     \mathcal{M}_{\phi}(X) = f(X) + \text{Lap}\left(\phi\right).
% \end{align*}
% % We'll now derive the data-dependent DP function $\epsilon_{\phi}(X)$ associated with $\mathcal{M}_{\phi}$:
% A rote calculation with the Laplace distribution tells us that
% \begin{align*}
%     \log \dfrac{\text{Pr}[\mathcal{M}_{\phi}(X) = y]}{\text{Pr}[\mathcal{M}_{\phi}(X') = y]} &\leq \dfrac{|f(X) - f(X')|}{\phi}.
% \end{align*}
% Using the above calculation and  Definition~\ref{def:data_dep_dp},
% \begin{align*}
%     \epsilon_{\phi}(X) = \max\limits_{X': X' \simeq X} \frac{|f(X) - f(X')|}{\phi} = \frac{\Delta_{LS}(X)}{\phi}.
% \end{align*}
% We can then verify that choosing $\phi = \beta/\hat{\epsilon}$ and $\hat{\epsilon} = \epsilon$ reduces Algorithm~\ref{alg:no_ls} exactly to Algorithm~\ref{alg:classic_ptr}.
% \end{example}
% \end{comment}



% \begin{remark}[Remove distance test]
% The distance test allows Example~\ref{exp: dist_ptr} to exploit properties of the local neighborhood of datasets close to the input dataset $X$. If $X$ is far away from the closest dataset whose local sensitivity or data-dependent DP exceeds the proposed bound, then $\gamma^P(X)$ will likely be quite large. The analogous condition in Example~\ref{exp: upperbound} to large distance $\gamma(X)$ is \emph{stable} data-dependent DP $\epsilon_{\phi, \hat{\delta}}(X)$. %Our caveat here is that
% % Example~\ref{exp: upperbound} works best for problems whose data-dependent DP has small sensitivity, or is parameterized by statistics  that have small sensitivity. 
% %-- a basic requirement (without which we would have zero utility) is $\Delta_{\phi} \leq \frac{\epsilon\hat{\epsilon}}{\log(1/\delta)}$. 
% \yw{I still don't understsand this remark. Remove?}
% \end{remark}

% Example~\ref{exp: upperbound} is more cautious than  Example~\ref{exp: dist_ptr} in the sense that if the data-dependent DP is at or just below the budget $\hat{\epsilon}$, then the test is more likely to produce a false negative which will cause the algorithm to output $\perp$. Fortunately, this downside is unlikely to manifest in the average case; the experimental results of \cite{redberg2021privately} indicate that instance-based privacy losses are often orders of magnitude smaller than the worst-case DP guarantee.
% \yw{The above paragraph confuses me more than it explains. If the data-dependent DP is at or just below, then the distance test will fail too?}
 



% In Section~\ref{sec: pate}, we demonstrate that one can upper bound the data-dependent DP through a modification of the smooth sensitivity framework applied on $\epsilon_\phi(X)$. Moreover, we provide a direct application of Example~\ref{exp: upperbound} with private linear regression by making use of the per-instance DP technique~\citep{wang2017per}. 



% \begin{comment}
% Moreover, if $\epsilon_\phi(X)$ admits a global sensitivity $\triangle_\phi$, we can use the tail bound of Laplace distribution for such a construction. \todo{Shall we mention privately release sufficient statistics here?}


% \begin{corollary}
% Assume that $\epsilon_\phi(X)$ has a global $L_1$ sensitivity $\triangle_\phi$. Let $\cT$ privately test if $\epsilon_{\phi, \hat{\delta}}^P(X) \leq \hat{\epsilon}$, where $\epsilon_{\phi,\hat{\delta}}^P(X):= \epsilon_{\phi, \hat{\delta}}(X)+ \text{Lap}(\frac{\triangle_
% \phi}{\epsilon}) + \frac{\triangle_\phi \log(1/\delta)}{\epsilon}$. Then an instantiation of Algorithm~\ref{alg:gen_ptr} with the test $\cT$ satisfies $(\epsilon+\hat{\epsilon}, \delta + \hat{\delta})$-DP.
% \end{corollary}
% \end{comment}



%\begin{theorem}
%Assume the data-dependent DP function of mechanism $\cM$
%satisfies $\epsilon_\phi(X)$ and its global $L_1$ sensitivity is bounded by $\triangle_\phi$. Then Algorithm~\ref{alg:no_dist} is $(\epsilon + \hat{\epsilon},\delta+\hat{\delta} )$-DP.
%\end{theorem}

 





% \begin{theorem}[\citep{wang2017per}]\label{thm: per}
% The algorithm used in Example~\ref{exp: posterior} with  parameter $(\lambda, \gamma)$ obeys $(\epsilon, \delta)$ data-dependent DP for each dataset $(X, \textbf{y})$  with 
% \[\epsilon = \sqrt{\frac{\gamma L^2 \log(2/\delta)}{\lambda + \lambda_{\min}}} + \frac{\gamma L^2}{2(\lambda + \lambda_{\min}+||\cX||^2)}+ \frac{1 + \log(2/\delta)||\cX||^2}{2(\lambda+\lambda_{\min})},
% \] where $L:=||\cX||(||\cX||||\theta_\lambda^*||+||\cY||)$ is the local Lipschitz constant, $\lambda_{\min}$ denotes the smallest eigenvalue of $X^TX$ and $||\theta_\lambda^*||$ is the magnitude of the solution $\theta_\lambda^* = (X^TX +\lambda I )^{-1}X^T \bf{y}$.
% \end{theorem}

% Notice that the data-dependent DP is a function of $(\lambda_{\min}, L, ||\theta_\lambda^*||, \lambda, \gamma)$, where $(\lambda_{\min}, L, ||\theta_\lambda^*||)$ are data-dependent quantities. One can apply the generalized PTR framework as in the following example.
% \begin{example} We demonstrate here how to apply generalized PTR to the one-posterior sample (OPS) algorithm, a differentially private mechanism which outputs one sample from the posterior distribution of a Bayesian model with bounded log-likelihood.
% \label{examp:ops}
% \begin{enumerate}\vspace{-1mm}
%     \item Propose $\phi=(\lambda, \gamma)$.\vspace{-1mm}
%     \item Based on $(\lambda, \gamma)$, differentially privately release $\lambda_{min}, ||\theta_\lambda^*||, L$ 
%     with privacy budget $(\epsilon, \delta/2)$.\vspace{-1mm}
%     \item Condition on a high probability event (with probability at least $1-\delta/2$) of $\lambda_{min}, ||\theta_\lambda^*||, L$, test if $\blue{\epsilon_{\phi}^P(X)}$  is smaller than the predefined privacy budget $(\hat{\epsilon}, \hat{\delta})$, where $\epsilon_\phi^P(X)$ denotes the sanitized data-dependent DP.\vspace{-1mm}
%     \item Based on the outcome of the test, decide whether to release $\theta \propto e^{-\frac{\gamma}{2}||\bf{y}-X\theta||^2 + \lambda||\theta||^2}$.\vspace{-1mm}
% \end{enumerate}
% \begin{theorem}
% The algorithm outlined in Example~\ref{examp:ops} satisfies $(\epsilon+ \hat{\epsilon}, \delta + \hat{\delta})$-DP. 
% \end{theorem}
% \end{example}


% The main idea of the above algorithm boils down to  privately releasing all data-dependent quantities in data-dependent DP, constructing high-probability confidence intervals of these quantities, and then deciding whether to run the mechanism $\cM$ with the proposed parameters. We defer the details of the privacy calibration of data-dependent quantities to the appendix. 

% One may ask why we cannot directly tune privacy parameters ($\lambda, \gamma$) based on the sanitized data-dependent DP. This is because, in many scenarios, data-dependent quantities depend on the choice of privacy parameters, e.g., $||\theta_\lambda^*||$ is a complicated function of $\lambda$. Thus, the optimization on $\lambda$ becomes a circular problem --- to solve $\lambda$, we need to sanitize $||\theta_
% \lambda^*||$, which needs to choose a $\lambda$ to begin with. Alternatively, generalized PTR provides a clear and flexible framework to test the validity of privacy parameters adapted to the dataset. 

% \begin{remark}
% The above ``circular'' issue is even more serious for generalized linear models (GLMs) beyond linear regression. The data-dependent DP there involves a local strong-convexity parameter, a complex function of the regularizer $\lambda$  and we only have zeroth-order access to. In the appendix, we demonstrate how to apply generalized PTR to provide a generic solution to a family of private GLMs where the link function satisfies a self-concordance assumption.
% \end{remark}
% \vspace{-2mm}

%we demonstrate that our generalized PTR provides a generic solution to private GLMs with data-adaptive analysis.
%In the appendix, we demonstrate that our generalized PTR can handle these cases effectively 
% in next selction, we demonstrate how we can combine the idea of privacy section for privacy calibration with the generalized PTR.




% remark it's close to sufficient statistic release. however, the data-dependent quantilties depends on the other parameters .


%We start by privately releasing $\lambda_{min}, L$ and $ ||\theta_\lambda^*||$ (condition on a high probability event). Then, the data-dependent DP is a function of $\phi = (\lambda, \gamma)$ with known global sensitivity $\triangle_\phi$. Next, we can apply Algorithm~\ref{alg:no_dist} to propose and test$(\lambda, \gamma)$ and decide whether to release $\theta \propto e^{-\frac{\gamma}{2}||\bf{y}-X\theta||^2 + \lambda||\theta||^2}$. We defer the full details to the appendix. 

==> Generalized PTR (1)/hyperparameter_selection.tex <==
This section introduces a method to jointly tune privacy parameters (e.g., noise scale) along with parameters related only to the utility of an algorithm (e.g., learning rate or batch size in stochastic gradient descent) -- while avoiding the $\perp$ output.

Algorithm~\ref{alg: parameter_ptr} takes a list of parameters as input, runs generalized PTR with each of the parameters, and returns the output with the best utility. We show that the privacy guarantee with respect to $\epsilon$ is independent of the number of $\phi$ that we try.  

Formally, let $\phi_1, ..., \phi_k$ be a set of hyper-parameters and $\tilde{\theta}_i \in\{\perp, \text{Range}(\cM)\}$ denotes the output of running generalized PTR on a private dataset $X$ with $\phi_i$. 
Let $X_{val}$ be a public validation set and $q(\tilde{\theta}_i)$ be the score of evaluating $\tilde{\theta}_i$ with $X_{val}$ (e.g., validation accuracy). The goal is to select a pair $(\tilde{\theta}_i$, $\phi_i)$ such that DP model $\tilde{\theta}_i$ maximizes the validation score.

The generalized PTR framework with privacy calibration is described in Algorithm~\ref{alg: parameter_ptr}. The privacy guarantee of Algorithm~\ref{alg: parameter_ptr} is an application of \citet{liu2019private}.


\begin{algorithm}[H]
	\caption{PTR with hyper-parameter selection}
	\label{alg: parameter_ptr}
	\begin{algorithmic}[1]
	   \STATE {\textbf{Input}:  Privacy budget per PTR algorithm ($\epsilon^*, \delta^*$), cut-off $T$, parameters $\phi_{1:k}$, flipping probability $\tau$ and validation score function $q(\cdot)$. } 
		\STATE {Initialize the set $S=\varnothing$.}
		\STATE{Draw $G$ from a geometric distribution $\cD_\tau$ and let $\hat{T}=\text{min}(T, G)$.}
		\FOR{i = 1 ,..., $\hat{T}$}
		\STATE{ pick a random $\phi_i$ from $\phi_{1:k}$.}
		\STATE{evaluate $\phi_i$: $(\tilde{\theta}_i, q(\tilde{\theta}_i))\gets$ Algorithm~\ref{alg:gen_ptr}($\phi_i, (\epsilon^*, \delta^*)$).}
		\STATE {$S \gets S \cup \{\tilde{\theta}_i, q(\tilde{\theta}_i)\}$.}
		%\STATE{with probability $\gamma$, we output the highest scored candidate from $S$ and halt.}
		\ENDFOR %\vspace{-1mm}
	\STATE{Output the highest scored candidate from $S$.}
	\end{algorithmic}
	%\vspace{-1mm}
\end{algorithm}

\begin{theorem}[ Theorem 3.4 \citet{liu2019private} ]
Fix any $\tau \in [0, 1], \delta_2>0$ and let $T =\frac{1}{\tau} \log \frac{1}{\delta_2}$. If each oracle access to Algorithm~\ref{alg:gen_ptr} is $(\epsilon^*, \delta^*)$-DP, then
Algorithm~\ref{alg: parameter_ptr} is $(3\epsilon^* + 3\sqrt{2\delta^*}, \sqrt{2\delta^*} T +\delta_2 )$-DP.%\yw{What if it does not reach $T$? Also in the algorithm it has $k$ right?  Also, did you define which score it is?}
\end{theorem}
The theorem implies that one can try a random number of $\phi$ while paying a constant $\epsilon$.
In practice, we can roughly set $\tau = \frac{1}{10k}$ so that the algorithm is likely to test all $k$ parameters. We emphasize that the privacy and the utility guarantee (stated in the appendix) is not our contribution. But the idea of applying generalized PTR to enforce a uniform DP guarantee over all choices of parameters with a data-dependent analysis is new, and in our opinion, significantly broadens the applicability to generic hyper-parameter tuning machinery from \citet{liu2019private}.

==> Generalized PTR (1)/introduction.tex <==
  %\vspace{-2em}
\section{Introduction}
   % \vspace{-1em}
\label{sec:introduction}
The guarantees of differential privacy (DP) \citep{dwork2006calibrating} are based on worst-case outcomes across all possible datasets. A common paradigm is therefore to add noise scaled by the \emph{global sensitivity} of a query $f$, i.e. the maximum change in $f$ between any pair of neighboring datasets.

A given dataset $X$ might have a \emph{local sensitivity} that is much smaller than the global sensitivity, in which case we can hope to add a smaller amount of noise (calibrated to the local rather than the global sensitivity) while achieving the same privacy guarantee. However, this must not be undertaken na\"{i}vely -- the local sensitivity is a dataset-dependent function and so calibrating noise to the local sensitivity could leak information about the dataset \citep{nissim2007smooth}.

The ``Propose-Test-Release'' (PTR) framework \citep{dwork2009differential} resolves this issue by introducing a test to privately check whether a proposed bound on the local sensitivity is valid. Only if the test ``passes'' is the output released with noise calibrated to the proposed bound on the local sensitivity. 

PTR is a powerful and flexible tool for designing data-adaptive DP algorithms, but it has several limitations. First, it applies only to noise-adding mechanisms which calibrate noise according to the sensitivity of a query. Second, the test in ``Propose-Test-Release'' is computationally expensive for all but a few simple queries such as privately releasing the median or mode.  Third, while some existing works\blue{~\citep{decarolis2020end, kasiviswanathan2013analyzing, liu2021differential}} follow the approach of testing ``nice'' properties of a dataset before exploiting these properties in a private release to PTR \footnote{We refer to these as PTR-like methods. }, 
there has not been a systematic recipe for \emph{discovering} which properties should be tested.
% \begin{enumerate}
%     \item It applies only to noise-adding mechanisms which calibrate noise according to the sensitivity of a query.
    
%     \item The test in ``Propose-Test-Release'' is computationally expensive for all but a few "nice" cases such as privately releasing the median or mode.
% \end{enumerate}

In this paper, we propose a generalization of PTR which addresses these limitations. The centerpiece of our framework is a differentially private test on the \emph{data-dependent privacy loss}.
%which meets a few requirements. 
This test does not directly consider the local sensitivity of a query and is therefore not limited to additive noise mechanisms. Moreover, in many cases, the test can be efficiently implemented by privately releasing a high-probability upper bound, thus avoiding the need to search an exponentially large space of datasets. Furthermore, the derivation of the test itself often spells out exactly what properties of the input dataset need to be checked, which streamlines the design of data-adaptive DP algorithms.

%Furthermore, the test need not search an exponentially large space of datasets and we illustrate how to design a test which privately checks requisite properties of the input dataset itself.


Our contributions are summarized as follows:
%\todo{to add }
\begin{enumerate}
    %\vspace{-1em}
    % \item We propose a generalization of PTR, which 
    % substantially broadens the applicability of the PTR framework \blue{on two fronts: (a) generalized PTR extends PTR to apply to any DP mechanisms (beyond noise-adding mechanisms); (b) generalized PTR allows us to plug in \emph{any} data-dependent DP analysis to construct a high-probability DP test that adapts to favorable properties of the input dataset -- without painstakingly designing each test from scratch.}
    \item We propose a generalization of PTR which can handle algorithms beyond noise-adding mechanisms. Generalized PTR allows us to plug in \emph{any} data-dependent DP analysis to construct a high-probability DP test that adapts to favorable properties of the input dataset -- without painstakingly designing each test from scratch.
   % \vspace{-0.7em}
    \item We demonstrate that many existing examples of PTR and PTR-like algorithms can be unified under the generalized PTR framework, sometimes resulting in a tighter analysis (see an example of report-noisy-max in Sec~\ref{sec:binary_vote}).   % \vspace{-0.7em}
    \item We show that one can publish a DP model through privately upper-bounding a one-dimensional statistic --- no matter how complex the output space of the mechanism is. We apply this result to solve an open problem from PATE \citep{papernot2017, papernot2018scalable}.    %\vspace{-1mm}
    \item Our results broaden the applicability of private hyper-parameter tuning \citep{liu2019private,papernot2021hyperparameter} in enabling joint-parameter selection of  DP-specific parameters (e.g., noise level) and native parameters of the algorithm (e.g., learning rate, regularization weight), which may jointly affect the data-dependent DP losses.    % \vspace{-0.7em}
\end{enumerate}

% \textbf{A remark on the DP test with case-specific study.}
% We concede that the data-dependent privacy loss might depend on the dataset in different ways, and thus the derivation of the test (used in the generalized PTR) requires a case-specific study. However, requiring a case-specific analysis for each problem seems to be a general problem that applies to all recipes for data-adaptive DP algorithm design. The required labor in the cases when standard PTR is applicable is equivalent to the work needed to derive and (privately) test the local sensitivity. When the classic PTR is not applicable, our framework provides a step-by-step guideline on what to do, which makes it more widely applicable.

% Moreover, we propose the following two approaches to construct the high-probability DP test.

% \begin{enumerate}
%     \item Private sufficient statistics release (used in the private linear regression example) specifies the data-dependent DP as a function of the dataset and privately releases each data-dependent component. 
%     \item The second approach (used in the PATE example) uses the smooth sensitivity framework to privately release the data-dependent DP as a whole, and then construct a high-confidence test using the Gaussian mechanism. 
    
% \end{enumerate}

% We believe these two approaches can cover most of the scenarios arising in data-adaptive analysis. For example, we demonstrate the merits of generalized PTR in handling data-adaptive private generalize linear models in the appendix using private sufficient statistics release. We believe this result is effective and not previously proposed in the literature. 
% Moreover, sufficient statistics release together with our private hyper-parameter tuning (Algorithm~\ref{alg: parameter_ptr} can be used to construct data-adaptive extensions of \blue{DP-PCA} and Sparse-DP-ERM (see details in the future work section).
% add citation

==> Generalized PTR (1)/local_sensitivity_examples.tex <==
Why do we want to generalize PTR beyond noise-adding mechanisms? Compared to classic PTR, the generalized PTR framework allows us to be more flexible in both the type of test conducted and also the type of mechanism whose output we wish to release. For many mechanisms, the local sensitivity either does not exist or is only defined for specific data-dependent quantities (e.g., the sensitivity of the score function in the exponential mechanism) rather than the mechanism's output. 

The following example illustrates this issue.

\begin{example}[Private posterior sampling]\label{exp: posterior}
Let $\cM: \cX\times \cY \to \Theta $ be a private posterior sampling   mechanism~\citep{minami2016differential,wang2015privacy,gopi2022private} for approximately minimizing $F_{X}(\theta)$.

$\cM$ samples $\theta \sim P(\theta)\propto e^{-\gamma(F_X(\theta)+ 0.5\lambda ||\theta||^2)}$ with parameters $\gamma, \lambda$. Note that $\gamma,\lambda$ cannot be appropriately chosen for this mechanism to satisfy DP without going through a sensitivity calculation of $\arg\min F_X(\theta)$. In fact, the global and local sensitivity of the minimizer is unbounded even in linear regression problems, i.e when $F_X(\theta) = \frac{1}{2}||y-X\theta||^2.$ 
%The local sensitivity $\Delta:=||P_{X,y}(\theta)-P_{X', y'}(\theta)||$ is not well-defined  for the sampling algorithm, thus the standard PTR is not applicable.  

\end{example}
Output perturbation algorithms do work for the above problem when we regularize, but they are known to be suboptimal in theory and in practice \citep{chaudhuri2011differentially}. In Section~\ref{subsections:private_linear_regression} we demonstrate how to apply generalized PTR to achieve a data-adaptive posterior sampling mechanism.

Even in the cases of noise-adding mechanisms where PTR seems to be applicable, it does not lead to a tight privacy guarantee. Specifically, by an example of privacy amplification by post-processing (Example~\ref{exp: binary_vote} in the appendix), we demonstrate that the local sensitivity does not capture all sufficient statistics for data-dependent privacy analysis and thus is loose.

% We've just seen an example where the local sensitivity is unbounded. In other cases, the local sensitivity exists and can be tested efficiently -- \emph{but} isn't sufficiently descriptive to make full use of data-dependent properties. Our next example demonstrates that considering only the local sensitivity leads to a loose privacy analysis.

% \begin{example}\label{exp: binary_vote}
% Consider a binary class voting problem: $n$ users vote for a binary class $\{0, 1\}$ and the goal is to output the class that is supported by the majority. Let $n_i$ denote the number of people who vote for the class $i$. We consider the report-noisy-max mechanism: $\cM(X): \text{argmax}_{i \in [0,1]} n_i(X)+ Lap(1/\epsilon)$,where $1/\epsilon$ denotes the scale of Laplace noise.

% For a dataset $X$, the gap between number of votes in each class is $t(X) = |n_0(X) - n_1(X)|$. Observe that if $t(X) > 1$, adding or removing one user will not change the majority class -- in other words, for a neighboring dataset $X'$ we have $\text{argmax}_{i \in [0,1]} n_i(X) = \text{argmax}_{i \in [0,1]} n_i(X')$. The local sensitivity $\Delta_{LS}(X)$ of the report-noisy-max mechanism is therefore $0$ if $t(X) >1$. 
% \end{example}

==> Generalized PTR (1)/pate.tex <==
%\vspace{-1em}
In this section, we apply the generalized PTR framework to solve an open problem from the Private Aggregation of Teacher Ensembles (PATE) \citep{papernot2017, papernot2018scalable} --- privately publishing the entire model through privately releasing data-dependent DP losses. Our algorithm makes use of the smooth sensitivity framework ~\citep{nissim2007smooth} and the Gaussian mechanism to construct a high-probability test of the data-dependent DP. The one-dimensional statistical nature of data-dependent DP enables efficient computations under the smooth sensitivity framework. Thus, this approach is generally applicable for other private data-adaptive analysis beyond PATE.

% shall we put this remark at the end of the section?


PATE  is a knowledge transfer framework for model-agnostic private learning. In this framework,  an ensemble of teacher models is trained on the disjoint private data and uses the teachers' aggregated consensus answers to supervise the training of a ``student'' model agnostic to the underlying machine-learning algorithms. By publishing only the aggregated answers and by the careful analysis of the ``consensus'', PATE has become a practical technique in recent private model training. 


The tight privacy guarantee of PATE heavily relies on a delicate data-dependent DP analysis, for which the authors of PATE use the smooth sensitivity framework  to privately publish the data-dependent privacy cost. However, it remains an open problem to show that the released model is DP under  data-dependent analysis. Our generalized PTR resolves this gap by  carefully testing a private upper bound of the data-dependent privacy cost. Our algorithm is fully described in Algorithm~\ref{alg: pate_ptr}, where the modification over the original PATE framework is highlighted in blue.


% put a pate framework here
 
Algorithm~\ref{alg: pate_ptr} takes the input of privacy budget $(\epsilon',\hat{\epsilon}, \delta)$, unlabeled public data $x_{1:T}$ and $K$ teachers' predictions on these data.  The parameter $\epsilon$ denotes the privacy cost of publishing the data-dependent DP and $\epsilon'$ is the predefined privacy budget for testing. $n_j(x_i)$ denotes the the number of teachers that agree on label $j$ for $x_i$ and $C$ denotes the number of classes. The goal is to privately release a list of plurality outcomes --- $\text{argmax}_{j\in[C]} n_j(x_i)$ for $i \in[T]$ --- and use these outcomes to supervise the training of a ``student'' model in the public domain. The parameter $\sigma_1$ denotes the noise scale for the vote count.


In their privacy analysis,  \citet{papernot2018scalable} compute the data-dependent $\rdp_{\sigma_1}(\alpha, X)$ of labeling the entire group of student queries.  $\rdp_{\sigma_1}(\alpha, X)$ can be orders of magnitude smaller than its data-independent version if there is a strong agreement among teachers. Note that $\rdp_{\sigma_1}(\alpha, X)$  is a function of the RDP order $\alpha$ and the dataset $X$, analogous to our  Definition~\ref{def:data_dep_dp}  but subject to RDP~\citep{mironov2017renyi}.
% We cite the comparison between two approaches for a special case.

\begin{theorem}[\citep{papernot2018scalable}]\label{thm: dep_gau}
If the top three vote counts of $x_i$ are $n_1>n_2>n_3$ and $n_1 -n_2, n_2-n_3\gg \sigma_1$, then the data-dependent RDP of releasing $\text{argmax}_j \{n_j +\cN(0, \sigma_1^2)\}$
satisfies $(\alpha, \exp\{-2\alpha/{\sigma_1^2}\}/\alpha)$-RDP and the data-independent RDP (using the Gaussian mechanism) satisfies $(\alpha, \frac{\alpha}{\sigma_1^2})$-RDP. 
\end{theorem}


\begin{algorithm}[H]
	\caption{PATE with generalized PTR}
	\label{alg: pate_ptr}
	\begin{algorithmic}[1]
		\STATE {\textbf{Input}: Unlabeled public data $x_{1:T}$, aggregated teachers prediction $n(\cdot)$, privacy parameter $\hat{\epsilon},\epsilon', \delta$, noisy parameter $\sigma_1.$}
		\STATE{Set  $\alpha =\frac{2\log(2/\delta)}{\hat{\epsilon}}+1 $, $\sigma_s = \sigma_2 = \sqrt{\frac{3\alpha + 2}{\hat{\epsilon}}}, \delta_2 = \delta/2, $ smoothness parameter $ \beta = \frac{0.2}{\alpha}$.}
		\STATE{Compute noisy labels: ${y_i}^p \gets \text{argmax}_{j\in [C]}\{n_j(x_i)+ \cN(0, \sigma_1^2)\} $ for all $i \in[1:T]$.}
		\STATE{$\rdp_{\sigma_1}(\alpha, X)\gets$ data-dependent RDP at the $\alpha$-th order.}
		\STATE {$SS_\beta(X) \gets$ the smooth sensitivity  of $\rdp_{\sigma_1}^{\text{upper}} (\alpha,X)$.}
		\STATE \blue{Privately release $\mu:=  \log(SS_\beta(X)) + \beta \cdot \cN(0, \sigma_2^2)+\sqrt{2\log(2/\delta_2)}\cdot \sigma_2 \cdot \beta$}
		\STATE{\blue{ $\rdp_{\sigma_1}^{\text{upper}}(\alpha)\gets $ an upper bound of data-dependent RDP through Lemma~\ref{lem: upperbound}}}.
		\STATE{\blue{$\epsilon_{\sigma_1} \gets$ DP guarantee converted from $\rdp_{\sigma_1}^{\text{upper}}(\alpha).$ }}
		%\gets \rdp_{\sigma_1} (\alpha, X)+ SS_{\beta}(X) \cdot \cN(0, \sigma_s^2)+ \blue{\sigma_s \cdot \sqrt{2\log(2/\delta_2)}e^{\mu} }+ \frac{\log(2/\delta)}{\alpha-1}$.}
		\STATE{\blue{If $\epsilon'\geq \epsilon_{\sigma_1}$ \textbf{return} a student model trained using $(x_{1:T}; y_{1:T}^p)$}}.
		\STATE{\blue{\text{Else return} $\perp$.}}
		%\STATE \blue{\textbf{if} $  \epsilon_{\sigma_1}(\alpha)^p + \frac{\log(2/\delta)}{\alpha-1} \leq \epsilon$ \textbf{return} a student model trained using $(x_{1:T}; y_{1:T}^p)$ \textbf{else return} $\perp.$}
	\end{algorithmic}
	%\vspace{-1mm}
\end{algorithm}



However, $\rdp_{\sigma_1}(\alpha, X)$ is data-dependent and thus cannot be revealed. The authors therefore privately publish the data-dependent RDP using the smooth sensitivity framework~\citep{nissim2007smooth}.
\begin{comment}
\begin{definition}[Smooth Sensitivity]\label{def: smooth}
	Given the smoothness parameter $\beta$, a $\beta$-smooth sensitivity of $f(X)$ is defined as 
	\[SS_\beta(X):= \max_{d\geq 0} e^{-\beta d} \cdot \max_{\tilde{X'}: dist(X, \tilde{X'})\leq d} \Delta_{LS}(\tilde{X}')\]
\end{definition}
\end{comment}
The smooth sensitivity calculates a smooth upper bound on the local sensitivity of $\rdp_{\sigma_1}(\alpha, X)$, denoted as $SS_\beta(X)$, such that $SS_\beta (X) \leq e^\beta SS_\beta(X')$ for any neighboring dataset $X$ and $X'$. By adding Gaussian noise scaled by the smooth sensitivity (i.e., release $\epsilon_{\sigma_1}(\alpha, X)+ SS_\beta(X)\cdot \cN(0, \sigma_s^2)$), the privacy cost is safely published. 


Unlike most noise-adding mechanisms, the standard deviation $\sigma_s$ cannot be published since $SS_\beta(X)$ is a data-dependent quantity. Moreover, this approach fails to provide a valid privacy guarantee of the noisy labels obtained through the PATE algorithm, as the published privacy cost could be smaller than the real privacy cost.
Our solution in Algorithm~\ref{alg: pate_ptr} looks like the following:
%\vspace{-2mm}
\begin{itemize}
    	%\vspace{-0.5em}
    \item Privately release an upper bound of the smooth sensitivity $SS_\beta(X)$ with $e^{\mu}$. % \vspace{-0.5em}
    \item Conditioned on a high-probability event of $e^{\mu}$, publish the data-dependent RDP with $\rdp_{\sigma_1}^{\text{upper}}(\alpha)$.
   % \vspace{-0.5em}
    \item Convert $\rdp_{\sigma_1}^{\text{upper}}(\alpha)$ back to the standard DP guarantee using RDP to DP conversion at $\delta/2$.  %\vspace{-0.5em}
    \item Test if the converted DP is above the predefined budget $\epsilon'$.
% \vspace{0.5em}
\end{itemize}
%\vspace{-2em}
The following lemma states that $\rdp_{\sigma_1}^{\text{upper}}(\alpha)$ is a valid upper bound of the data-dependent RDP.

\begin{figure*}[t]
	\centering	
	\subfigure[High consensus and strong data-dependent DP ]{
	\includegraphics[width=0.46\textwidth]{img/pate_high.pdf}\label{fig:high}}
	\subfigure[Low consensus and low data-dependent DP]{
	\includegraphics[width=0.46\textwidth]{img/pate_low.pdf}\label{fig:low}} %\vspace{-3mm}
	\caption{Privacy and utility tradeoffs with PATE. 
	When $\sigma_1$ is aligned, three algorithms provide the same utility. $y$-axis plots the privacy cost of labeling $T=200$ public data with $\delta = 10^{-5}$.
   The left figure considers the high-consensus case, where the data-adaptive analysis is preferred.} 
	\label{fig: exp_pate}
	%\vspace{-1em}
\end{figure*}

\begin{lemma}[Private upper bound of data-dependent  RDP]\label{lem: upperbound}
We are given a RDP function $\rdp(\alpha, X)$ and a $\beta$-smooth sensitivity bound $SS(\cdot)$ of $\rdp(\alpha, X)$. Let $\mu$ (defined in Algorithm~\ref{alg: pate_ptr}) denote the private release of $\log(SS_\beta(X))$. Let the $(\beta, \sigma_s, \sigma_2)$-GNSS mechanism be 
\[\scriptstyle
\rdp^{\text{upper}}(\alpha):=\rdp(\alpha, X) + SS_\beta(X) \cdot \cN(0, \sigma_s^2) + \sigma_s \sqrt{2\log(\frac{2}{\delta_2}) } e^{\mu} \]
	 Then, the release of $\rdp^{\text{upper}}(X)$ satisfies $(\alpha, \frac{3\alpha +2}{2\sigma_s^2})$-RDP for all $1<\alpha < \frac{1}{2\beta}$; w.p. at least $1-\delta_2$, $\rdp^{\text{upper}}(\alpha)$ is an upper bound of $\rdp(\alpha, X)$.
%\vspace{-2mm}
\end{lemma}


The proof (deferred to the appendix) makes use of the facts that: (1) the log of $SS_\beta(X)$ has a bounded global sensitivity $\beta$ through the definition of smooth sensitivity; (2) releasing $\rdp_{\sigma_1}(\alpha, X)+ SS_\beta(X)\cdot \cN(0, \sigma_s^2)$ is $(\alpha, \frac{\alpha+1}{\sigma_s^2})$-RDP (Theorem 23 from \citet{papernot2018scalable}).

%The theorem provides a universal solution to sani any smooth sensitivity based data-dependent DP.
% remark, the theorem provides a general approach

%Next, we convert $\epsilon_{\sigma_1}(\alpha)^p$ back to the standard DP guarantee, and compare it with the pre-defined privacy budget $\epsilon$. Once the test passes, Algorithm~\ref{alg: pate_ptr} returns the noise parameter as well as the noisy aggregated labels.


Now, we are ready to state the privacy guarantee of Algorithm~\ref{alg: pate_ptr}.





\begin{theorem}\label{thm: pate_ptr}
Algorithm~\ref{alg: pate_ptr} satisfies $(\epsilon'+\hat{\epsilon}, \delta)$-DP.
\end{theorem}
%\vspace{-2mm}
%short version
In the proof, the choice of $\alpha$ ensures that the cost of the $\delta/2$ contribution (used in the RDP-to-DP conversion) is roughly $\hat{\epsilon}/2$. Then  the release of $\rdp_{\sigma_1}^{\text{upper}}(\alpha)$ with  $\sigma_s =\sqrt{\frac{2+3\alpha}{\hat{\epsilon}}}$ accounts for another cost of $(\epsilon/2, \delta/2)$-DP.% Finally, the testing step is $\epsilon$-DP.

%In the proof, we set $\alpha =\frac{2\log(2/\delta)}{\epsilon}+1$ and use RDP to DP conversion with $\delta/2$ ensures that the cost of $\delta/2$ contribution to be roughly $\epsilon/2$. Then, the release of $\epsilon_{\sigma_1}^p(\alpha)$ with  $\sigma_s =\sqrt{\frac{2+3\alpha}{\epsilon}}$ counts for another $(\epsilon/2, \delta/2)$-DP.


%Regarding the  practical choice on $\epsilon$, we can set 
%$\epsilon = \frac{1}{4}\bigg(\frac{T}{\sigma_1^2}+2\sqrt{\frac{T\log(1/\delta)}{\sigma_1^2}}\bigg)$ (a quarter of the data-independent cost), so that the algorithm returns $\perp$ only when the data-dependent DP is close to its data-independent version.  Alternatively, we provide a no-$\perp$ version of Algorithm~\ref{alg: pate_ptr} by removing its testing step, which satisfies $(\epsilon_{\sigma_1}(\alpha)^p + \epsilon, \delta)$-DP. 

\textbf{Empirical results.} We next empirically evaluate Algorithm~\ref{alg: pate_ptr} (PATE-PTR) on the MNIST dataset. Following the experimental setup from \citet{papernot2018scalable}, we consider the training set to be the private domain, and the testing set is used as the public domain.  We first partition the training set into $400$ disjoint sets and $400$ teacher models, each trained individually. Then we select $T=200$ unlabeled data from the public domain, with the goal of privately labeling them. 
To illustrate the behaviors of algorithms under various data distributions, we consider two settings of unlabeled data, high-consensus and low-consensus. In the low-consensus setting, we choose $T$ unlabeled data such that there is no high agreement among teachers, so the advantage of data-adaptive analysis is diminished. We provide further details on the distribution of these two settings in the appendix.
%In the low-consensus setting, we apply a screening on public data and only use data whose maximum vote count is smaller than $150$, so the advantage of data-adaptive analysis is diminished. We provide the distribution of two settings in the appendix.
% mention how to compute the smooth sensitivity

\textbf{Baselines.}
We consider the Gaussian mechanism as a data-independent baseline, where the privacy guarantee is valid but does not take advantage of the properties of the dataset. The data-dependent DP (~\citet{papernot2018scalable}) serves as a non-private baseline, which requires further sanitation.  Note that these two baselines provide different privacy analyses of the same algorithm (see Theorem~\ref{thm: dep_gau}).




Figure~\ref{fig: exp_pate} plots privacy-utility tradeoffs between the three approaches by varying the noise scale $\sigma_1$. The purple region denotes a set of privacy budget choices ($\hat{\epsilon}+\epsilon'$ used in Algorithm~\ref{alg: pate_ptr}) such that the utility of the three algorithms is aligned under the same $\sigma_1$. In more detail, the purple region is lower-bounded by $\hat{\epsilon} +\epsilon_{\sigma_1}$.
We first fix $\sigma_s=\sigma_2=15$ such that $\hat{\epsilon}$ is fixed. Then we empirically calculate the average of $\epsilon_{\sigma_1}$ (the private upper bound of the data-dependent DP) over $10$ trials. Running Algorithm~\ref{alg: pate_ptr} with any choice of $\hat{\epsilon}+\epsilon'$ chosen from the purple region implies  $\epsilon'>\epsilon_{\sigma_1}$. Therefore, PATE-PTR will output the same noisy labels (with high probability) as the two baselines.


\textbf{Observation} 
As $\sigma_1$ increases, the privacy loss of the Gaussian mechanism decreases, while the data-dependent DP curve does not change much. This is because the data-dependent DP of each query is a complex function of both the noise scale and the data and does not monotonically decrease when $\sigma_1$ increases (see more details in the appendix). However, the data-dependent DP still dominates the Gaussian mechanism for a wide range of $\sigma_1$. Moreover, PATE-PTR nicely interpolates between the data-independent DP guarantee and the non-private data-adaptive DP guarantee.  In the low-consensus case, the gap between the data-dependent DP and the DP guarantee of the Gaussian mechanism unsurprisingly decreases. Meanwhile, PATE-PTR (the purple region) performs well when the noise scale is small but deteriorates when the data-independent approach proves more advantageous. 
This example demonstrates that using PTR as a post-processing step to convert the data-dependent DP to standard DP is effective when the data-adaptive approach dominates others.





 %Figure~\ref{fig: exp_pate} plots privacy-utility tradeoffs between three approaches by varying noisy scale $\sigma_1$. As $\sigma_1$ increases, the privacy loss of  Gaussian mechanism decreases, while the curve of data-dependent DP does not change much. This is because the data-dependent DP of each query is a function of $q$, where $q$ denotes an upper bound of the probability where the plurality output does not match the noisy output. $q$ is a complex function of both the noisy scale and data and is not monotonically decreasing when $\sigma_1$ is increasing. 









==> Generalized PTR (1)/preliminary.tex <==
%\vspace{-1em}
\section{Preliminaries}
%\vspace{-1em}
\label{sec:preliminaries}
Datasets $X, X' \in \mathcal{X}$ are neighbors if they differ by no more than one datapoint -- i.e., $X \simeq X'$ if $d(X, X') \leq 1$. We will define $d(\cdot)$ to be the number of coordinates that differ between two datasets of the same size $n$: $d(X, Y) = \#\{i \in [n]: X_i \neq Y_i  \}$.

We use $||\cdot||$ to denote the radius of the smallest Euclidean ball that contains the input set, e.g. $||\mathcal{X}|| = \sup_{x \in \mathcal{X}} ||x||$.

The parameter $\phi$ denotes the privacy parameters associated with a mechanism (e.g. noise level, regularization). $\mathcal{M}_{\phi}$ is a mechanism parameterized by $\phi$.
For mechanisms with continuous output space, we will take $\text{Pr}[\mathcal{M}(X) = y]$ to be the probability density function of $\mathcal{M}(X)$ at $y$.



    \begin{definition}[Differential privacy \citep{dwork2006calibrating}] \label{def:dp}
        Fix $\epsilon, \delta \geq 0$. 
A randomized algorithm $\mathcal{M}: \mathcal{X} \rightarrow \mathcal{S}$ satisfies $(\epsilon, \delta)$-DP if for all neighboring datasets $X \simeq X'$ and for all measurable sets $S \subset \mathcal{S}$, 
            \[\text{Pr}\big[\mathcal{M}(X) \in S\big] \leq e^{\epsilon}\text{Pr}\big[\mathcal{M}(X') \in S\big] + \delta.\]
    \end{definition}
%\vspace{-3mm}
% We now define \emph{data-dependent} differential privacy that conditions on an input dataset $X$. 

% \begin{definition}[Data-dependent privacy\cite{papernot2018scalable}]\vspace{-1mm}
% \label{def:data_dep_dp}
% Suppose we have $\delta > 0$ and a function $\epsilon: \mathcal{X} \rightarrow \mathbb{R}$. We say that mechanism $\mathcal{M}$ satisfies ($\epsilon(X), \delta$) data-dependent DP for dataset $X$ if for all possible output sets $S$ and neighboring datasets $X'$,
% \begin{align*}
%     \text{Pr}\big[\mathcal{M}(X) \in S\big] &\leq e^{\epsilon(X)}\text{Pr}\big[\mathcal{M}(X') \in S\big] + \delta, \\
%       \text{Pr}\big[\mathcal{M}(X') \in S\big] &\leq e^{\epsilon(X)}\text{Pr}\big[\mathcal{M}(X) \in S\big] + \delta.
% \end{align*}
% \end{definition}

%\subsection{Additive Noise Mechanisms}
Suppose we wish to privately release the output of a real-valued function $f: \mathcal{X} \rightarrow \mathcal{R}$. We can do so by calculating the \emph{global sensitivity} $\Delta_{GS}$, calibrating the noise scale to the global sensitivity and then adding sampled noise to the output.



\begin{definition}[Local / Global sensitivity]
The local $\ell_*$-sensitivity of a function $f$ is defined as $\Delta_{LS}(X) = \max\limits_{X \simeq X'} || f(X) - f(X') ||_* $ and the global sensitivity of $f$ is $\Delta_{GS} = \sup_X \Delta_{LS}(X)$.
% The local $\ell_*$-sensitivity of a function $f: \cX \to \mathbb{R}^d$ is defined as $\Delta_{LS}(X) = \max\limits_{X \simeq X'} || f(X) - f(X') ||_* $ and the global sensitivity of $f$ is $\Delta_{GS} = \sup_X \Delta_{LS}(X)$.
\end{definition}
%\vspace{-2mm}
% The choice of $\ell_*$ depends on which kind of noise we use, e.g., $\ell_2$-norm is used for Gaussian noise.

\begin{comment}

\begin{definition}[Global sensitivity]
The global $\ell_*$-sensitivity of a function $f: \mathcal{X} \rightarrow \mathcal{R}^d$ is defined as
\begin{align*}
    \Delta_{GS} &= \max\limits_{X, X' \in \mathcal{X}:X \simeq X'} || f(X) - f(X') ||_*. 
\end{align*}
\end{definition}
\begin{definition}[Laplace mechanism]
The Laplace mechanism $\mathcal{M}: \mathcal{X} \rightarrow \mathbb{R}$ applied to a function $f$ is given as
\begin{align*}
    \mathcal{M}(X) &= f(X) + \text{Lap}\left(b \right).
\end{align*}
\end{definition}
\begin{theorem}
Suppose the function $f: \mathcal{X} \rightarrow \mathbb{R}$ has global $\ell_1$-sensitivity $\Delta_f$. Then the Laplace mechanism satisfies $\epsilon$-differential privacy with noise parameter $b = \Delta_f/\epsilon$.	 \vspace{-2mm}
\end{theorem}

\begin{definition}[Gaussian mechanism]
The Gaussian mechanism $\mathcal{M}: \mathcal{X} \rightarrow \mathbb{R}$ applied to a function $f$ is given as
\begin{align*}
    \mathcal{M}(X) &= f(X) + \mathcal{N}(0, \sigma^2).
\end{align*}
\end{definition}
\begin{theorem}
Suppose the function $f: \mathcal{X} \rightarrow \mathbb{R}$ has global $\ell_2$-sensitivity $\Delta_f$. Then the Gaussian mechanism satisfies $(\epsilon, \delta)$-differential privacy with noise parameter $\sigma = \Delta_f\sqrt{2 \log(1.25/\delta)}/\epsilon$.
\end{theorem}
Both the Laplace and Gaussian mechanisms generalize easily to releasing the output of a $d$-dimensional function $f$ by adding i.i.d. noise to each coordinate.
\begin{definition}[Local sensitivity]
The local $\ell_*$-sensitivity of a function $f: \mathcal{X} \rightarrow \mathbb{R}^d$ is defined as
\begin{align*}
    \Delta_{LS}(X) &= \max\limits_{X \simeq X'} || f(X) - f(X') ||_*. 
\end{align*}
\end{definition}
\end{comment}
% \todo{Define Global sensitivity}
%define global/local sensitivity
%Laplace, Gaussian mech
% explain how related to PTR and its generalization

%\vspace{-0.em}
\subsection{Propose-Test-Release}
%\vspace{-0.5em}
Calibrating the noise level to the local sensitivity $\Delta_{LS}(X)$ of a function would allow us to add less noise and therefore achieve higher utility for releasing private queries. However, the local sensitivity is a data-dependent function and na\"ively calibrating the noise level to $\Delta_{LS}(X)$ will not satisfy DP.

PTR resolves this issue in a three-step procedure: \textbf{propose} a bound on the local sensitivity, privately \textbf{test} that the bound is valid (with high probability), and if so calibrate noise according to the bound and \textbf{release} the output.

% \begin{figure}[t]
% \vspace{-1em}
% \centering
% \resizebox{0.95\columnwidth}{!}{%
% \begin{minipage}{0.50\textwidth}
% \begin{algorithm}[H]
% \caption{Propose-Test-Release \cite{dwork2009differential}}
% \label{alg:classic_ptr}
% \begin{algorithmic}[1]
% \STATE{\textbf{Input}: Dataset $X$; privacy parameters $\epsilon,\delta$; proposed bound $\beta$ on $\Delta_{LS}(X)$; query function $f: \mathcal{X} \rightarrow \mathbb{R}$.}
% \STATE{\textbf{Output}: $f^P(X)$ or $\perp$.}
% \STATE{Compute the distance $\gamma(X)$ to the nearest dataset $X''$ such that $ \Delta_{LS}(X'')> \beta$:
% $\gamma(X) = \min\limits_{X''} \{ \text{dist}(X, X''): \Delta_{LS}(X'')> \beta \}$.}
% \STATE{Privately release $\gamma^P(X) = \gamma(X) + \text{Lap}\left(\frac{1}{\epsilon}\right)$.}
% \IF{$\gamma^P(X) > \dfrac{\log(1/\delta)}{\epsilon}$}\vspace{-1pt}
% \STATE{Release $f^P(X) = f(X) + \text{Lap}\left(\frac{\beta}{\epsilon}\right)$.}\vspace{-2pt}
% \ELSE
% \STATE{Output $\perp$.}\vspace{-1pt}
% \ENDIF
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \quad
% \begin{minipage}{0.46\textwidth}
% \begin{algorithm}[H]
% \caption{Generalized PTR}
% \label{alg:gen_ptr}
% \begin{algorithmic}[1]
% \STATE{{Input}: Proposed~parameter~$\phi$;~privacy~parameters~$\epsilon,  \hat{\epsilon}, \hat{\delta}$; dataset $X$;\blue{an $(\epsilon,\delta)$~DP test $\cT$; ~data-dependent~DP~function~$\epsilon_{\phi}(\cdot, \hat{\delta})$;~mechanism~$\mathcal{M}_{\phi}$.}}
% \STATE{\textbf{Output}: 
% $\mathcal{M}_{\phi}(X)$ or $\perp$.}
% \STATE{Let $\cT$ privately test if $\epsilon_\phi(X,\hat{\delta}) \leq \hat{\epsilon}$.}% with privacy limit $(\hat{\epsilon}, \hat{\delta})$ }.
% \IF{the test $\cT$ passes}
% \vspace{1pt}
% \STATE{Run $\theta = \mathcal{M}_{\phi}(X)$ and output $\theta$.}\vspace{2pt}

% \ELSE \vspace{2pt}

% \STATE{Output $\perp$.}\vspace{2pt}

% \ENDIF
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% }
% \vspace{-1em}
% \end{figure}


% \begin{theorem} 
% Algorithm~\ref{alg:classic_ptr} satisfies ($2 \epsilon, \delta$)-DP.
% \cite{dwork2009differential}
% \end{theorem}

PTR privately computes the distance $\cD_{\beta}(X)$ between the input dataset $X$ and the nearest dataset $X''$ whose local sensitivity exceeds the proposed bound $\beta$:
\begin{align*}
    \cD_{\beta}(X) = \min\limits_{X''} \{ d(X, X''): \Delta_{LS}(X'')> \beta \}.
\end{align*}
%\vspace{-.8em}
% The $\epsilon$-DP "test" fails (with probability $\delta$) if PTR decides to release $f^P(X)$ when $\gamma(X) = 0$, i.e. when dataset $X$ has local sensitivity greater than $\beta$.

\begin{figure}[H]
\vspace{-1.4em}
\centering
% \resizebox{0.95\columnwidth}{!}{%
% \begin{minipage}{0.54\textwidth}
\begin{algorithm}[H]
\caption{Propose-Test-Release \citep{dwork2009differential}}
\label{alg:classic_ptr}
\begin{algorithmic}[1]
\STATE{\textbf{Input}: Dataset $X$; privacy parameters $\epsilon,\delta$; proposed bound $\beta$ on $\Delta_{LS}(X)$; query function $f: \mathcal{X} \rightarrow \mathbb{R}$.}
% \STATE{\textbf{Output}: $f^P(X)$ or $\perp$.}
% \STATE{Compute the distance $\gamma(X)$ to the nearest dataset $X''$ such that $ \Delta_{LS}(X'')> \beta$.}
% \STATE{Privately release $\gamma^P = \gamma(X; \beta) + \text{Lap}\left(\frac{1}{\epsilon}\right)$.}

\STATE{\textbf{if} $\cD_{\beta}(X) + \text{Lap}\left(\frac{1}{\epsilon}\right) \leq \frac{\log(1/\delta)}{\epsilon}$ \textbf{then} output $\perp$,}
\STATE{\textbf{else} release $f(X) + \text{Lap}\left(\frac{\beta}{\epsilon}\right)$.}
\end{algorithmic}
\end{algorithm}
\end{figure}
%\vspace{-.8em}
\begin{theorem} 
Algorithm~\ref{alg:classic_ptr} satisfies ($2 \epsilon, \delta$)-DP.
\citep{dwork2009differential}
\end{theorem}
%\vspace{-1em}
Rather than proposing an arbitrary threshold $\beta$, one can also privately release an upper bound of the local sensitivity and calibrate noise according to this upper bound. This was used for node DP in graph statistics \citep{kasiviswanathan2013analyzing}, and for fitting topic models using spectral methods \citep{decarolis2020end}.

%This gives a more efficient alternative and avoids the need to propose $\beta$. This variant is  the local sensitivity itself has a global sensitivity.

%there exist other variants of PTR --- e.g., compute a differentially private upper bound of the local sensitivity and calibrate noise according to this upper bound. This type of PTR requires a global sensitivity of the local sensitivity. We refer readers to the excellent summary of PTR in  section 3 of \citet{vadhan2017complexity}.

% We may mention other types of PTR: propose and release
% There are other variants of PTR... 
% \vspace{-1mm}
% \subsection{Motivation}
% \vspace{-1mm}
% Why do we want to generalize PTR beyond noise-adding mechanisms? For other mechanisms, the local sensitivity either does not exist or is only defined for specific data-dependent quantities (e.g., the sensitivity of the score function in the exponential mechanism) rather than the mechanism's output. We give a concrete example below. 

%In this section, we give a concrete example to demonstrate this limitation and motivate our generalization.
%This section discusses a few limitations of PTR approaches that motivated our work.
%Let us first ask, ``is PTR a general framework applicable to any mechanism with a data-dependent analysis?'' If so, we could explore other less costly approaches to privately test the local sensitivity.

%However, the answer is unfortunately ``no''.  The reasons are twofold. First, the framework above applies only to ``noise-adding'' mechanisms --- where we have a well-defined local sensitivity (of the output), and the noise scale is calibrated according to that. For other non-noise-adding mechanisms, the local sensitivity either does not exist or is only defined for specific data-dependent quantities (e.g., the sensitivity of the score function in the exponential mechanism) rather than the mechanism's output. Consider the difficulties of applying PTR to the following example.


% \begin{example}[Private posterior sampling]\label{exp: posterior}
% Let $\cM: \cX\times \cY \to \Theta $ be a private posterior sampling   mechanism~\citep{minami2016differential,wang2015privacy,gopi2022private} for approximately minimizing $F_{X}(\theta)$. % for linear regression problem, i.e., $\min_{\theta} \frac{1}{2}||y-X\theta||^2 + \lambda ||\theta||^2$. 
% $\cM$ samples $\theta \sim P(\theta)\propto e^{-\gamma(F_X(\theta)+ 0.5\lambda ||\theta||^2)}$ with parameters $\gamma, \lambda$. $\gamma,\lambda$ cannot be appropriately chosen for this mechanism to satisfy DP without going through a sensitivity calculation of $\arg\min F_X(\theta)$. In fact, the global and local sensitivity of the minimizer is unbounded even in linear regression problems, i.e., when $F_X(\theta) = \frac{1}{2}||y-X\theta||^2.$ 
% %The local sensitivity $\Delta:=||P_{X,y}(\theta)-P_{X', y'}(\theta)||$ is not well-defined  for the sampling algorithm, thus the standard PTR is not applicable.  
% \end{example}
% Output perturbation algorithms do work for the above problem when we regularize, but they are known to be suboptimal in theory and in practice \cite{chaudhuri2011differentially}.% do not achieve the level of utility in theory and in practice when comparing to posterior sampling. 
 

% Moreover, even in the cases of noise-adding mechanisms where PTR seems to be applicable, it does not lead to a tight privacy guarantee. Specifically, by an example of privacy amplification by post-processing (Example~\ref{exp: binary_vote} in the appendix), we demonstrate that the local sensitivity does not capture all sufficient statistics for data-dependent privacy analysis and thus is loose.

% Instead of identifying sufficient statistics of each mechanism, we develop a unified framework --- generalized PTR, offering the flexibility for any mechanism to exploit data-dependent quantities.

% \textbf{On data-dependent DP losses.} In addition to the above, there has been an increasing list of empirical DP work that fix the parameters of a randomized algorithm while reporting the resulting data-dependent DP losses $\epsilon(\text{Data})$ after running on a specific dataset \citep{ligett2017accuracy,papernot2018scalable,zhu2020private, feldman2021individual}. The data-dependent DP losses are often smaller than the worst-case DP losses, but technically speaking, these algorithms are not formally DP with DP guarantees any smaller than that of the worst-case. In addition, the data-dependent DP losses themselves are sensitive, and thus cannot be reported. A typical solution is to privately release $\epsilon(\text{Data})$, but it still does not satisfy DP as this would require a prescribed $(\epsilon,\delta)$-DP parameter to be satisfied for all input datasets. Part of our contribution is to resolve this conundrum by showing that a simple post-processing step of the privately released upper bound of $\epsilon(\text{Data})$ gives a formal DP algorithm.
%\yq{Shall we combine this part with the related work section?}

%Instead,  exploits data-dependent quantities by first privately choosing $\gamma, \lambda$ adapted to the dataset and then applying posterior sampling with the sanitized parameters.  


==> Generalized PTR (1)/private_linear_regression.tex <==
\begin{figure*}[t]
	\centering	
	\subfigure[Bike dataset]{
	\includegraphics[width=0.48\textwidth]{img/bike.pdf}\label{fig:bike}}
	\subfigure[Elevators dataset]{
	\includegraphics[width=0.46\textwidth]{img/elevator.pdf}\label{fig:ele}}
	%\vspace{-0.5em}
	\caption{Differentially private linear regression algorithms on UCI datasets. $y$-axis reports the MSE error with confidence intervals. $\epsilon$ is evaluated with $\delta = 1e-6$. }
	\label{fig:selection}%\vspace{-0.5em}
\end{figure*}



\begin{theorem}[\citep{wang2017per}]\label{thm: per}
For input data $X \in \mathcal{X}$ and $Y \in \mathcal{Y}$, define the following:
\begin{itemize}
    %\vspace{-1em}
    \item $\lambda_{\min}(X)$ denotes the smallest eigenvalue of $X^TX$; %\vspace{-1em}
    \item $||\theta_\lambda^*||$ is the magnitude of the solution $\theta_\lambda^* = (X^TX +\lambda I )^{-1}X^T Y$;%\vspace{-1em}
    \item and $L(X, \mathbf{y}):=||\cX||(||\cX||||\theta_\lambda^*||+||\cY||)$ is the local Lipschitz constant, denoted $L$ in brief.%\vspace{-1em}
\end{itemize}
For brevity, denote $\lambda^* = \lambda + \lambda_{\min}(X)$.
The algorithm used in Example~\ref{exp: posterior} with  parameter $\phi = (\lambda, \gamma)$ obeys $(\epsilon_{\phi}(Z), \delta)$ data-dependent DP for each dataset $ Z = (X, Y)$  with $\epsilon_{\phi}(Z)$ equal to
\[\sqrt{\frac{\gamma L^2 \log(2/\delta)}{\lambda^*}} + \frac{\gamma L^2}{2(\lambda^*  +||\cX||^2)}+ \frac{1 + \log(2/\delta)||\cX||^2}{2(\lambda^*)}.
\]
\end{theorem}

Notice that the data-dependent DP is a function of $(\lambda_{\min}, L, ||\theta_\lambda^*||, \lambda, \gamma)$, where $(\lambda_{\min}, L, ||\theta_\lambda^*||)$ are data-dependent quantities. One can apply the generalized PTR framework as in the following example.
\begin{example}[OPS with PTR] We demonstrate here how to apply generalized PTR to the one-posterior sample (OPS) algorithm, a differentially private mechanism which outputs one sample from the posterior distribution of a Bayesian model with bounded log-likelihood.
\label{examp:ops}
\begin{itemize}
    %\vspace{-1em}
    \item Propose $\phi=(\lambda, \gamma)$.    %\vspace{-0.5em}
    \item Based on $(\lambda, \gamma)$, differentially privately release $\lambda_{min}, ||\theta_\lambda^*||, L$ 
    with privacy budget $(\epsilon, \delta/2)$.    %\vspace{-0.5em}
    \item Condition on a high probability event (with probability at least $1-\delta/2$) of $\lambda_{min}, ||\theta_\lambda^*||, L$, test if $\blue{\epsilon_{\phi}^P(X)}$  is smaller than the predefined privacy budget $(\hat{\epsilon}, \hat{\delta})$, where $\epsilon_\phi^P(X)$ denotes the sanitized data-dependent DP.   % \vspace{-1em}
    \item Based on the outcome of the test, decide whether to release $\theta \propto e^{-\frac{\gamma}{2}||Y-X\theta||^2 + \lambda||\theta||^2}$.   % \vspace{-1em}
\end{itemize}
\begin{theorem}
The algorithm outlined in Example~\ref{examp:ops} satisfies $(\epsilon+ \hat{\epsilon}, \delta + \hat{\delta})$-DP. 
\end{theorem}
\end{example}

%\vspace{-0.5em}
The main idea of the above algorithm boils down to  privately releasing all data-dependent quantities in data-dependent DP, constructing high-probability confidence intervals of these quantities, and then deciding whether to run the mechanism $\cM$ with the proposed parameters. We defer the details of the privacy calibration of data-dependent quantities to the appendix. 

One may ask why we cannot directly tune privacy parameters ($\lambda, \gamma$) based on the sanitized data-dependent DP. This is because, in many scenarios, data-dependent quantities depend on the choice of privacy parameters, e.g., $||\theta_\lambda^*||$ is a complicated function of $\lambda$. Thus, the optimization on $\lambda$ becomes a circular problem --- to solve $\lambda$, we need to sanitize $||\theta_
\lambda^*||$, which needs to choose a $\lambda$ to begin with. Alternatively, generalized PTR provides a clear and flexible framework to test the validity of privacy parameters adapted to the dataset. 

\begin{remark}
The above ``circular'' issue is even more serious for generalized linear models (GLMs) beyond linear regression. The data-dependent DP there involves a local strong-convexity parameter, a complex function of the regularizer $\lambda$  and we only have zeroth-order access to. In the appendix, we demonstrate how to apply generalized PTR to provide a generic solution to a family of private GLMs where the link function satisfies a self-concordance assumption.
\end{remark}
%\vspace{-0.5em}

We next apply Algorithm~\ref{alg: parameter_ptr} for Example~\ref{examp:ops}  with UCI regression datasets. Standard z-scoring is applied and each data point is normalize with a Euclidean norm of 1.  We consider $(60\%,10\%,30\%)$ splits for training, validation and testing test.

\textbf{Baselines}
\begin{itemize}
%\vspace{-0.5em}
    \item Output Perturbation (Outpert)~\citep{chaudhuri2011differentially}: $\theta=(X^TX + \lambda I)^{-1}X^T\bf{y}$. Release $\hat{\theta} = \theta + \bf{b}$ with an appropriate $\lambda$, where $\bf{b}$ is a Gaussian random vector.%\vspace{-1em}
    \item Posterior sampling (OPS). Sample $\hat{\theta}\sim P(\theta)\propto e^{-\gamma(F(\theta)+ 0.5 \lambda ||\theta||^2)}$ with parameters $\gamma, \lambda$.%\vspace{-1em}
    \item Adaptive posterior sampling (AdaOPS)~\citep{wang2018revisiting}. Run OPS with $(\lambda, \gamma)$ chosen adaptively according to the dataset.%\vspace{-1em}
\end{itemize}
%\yw{\cite{gopi2022private} had a nice and clean Gaussian DP bound for OPS. I thought if we can privately test the strong convexity from the dataset, it should satisfy a stronger Gaussian DP. How are privacy accounted in the experiments now?} % use composition.  Each oracle call is (eps, delta). split (epsilon/2, delta/2) to release data dependent quantity, use the remaining to tune gamma for an input lambda.
Outpert and OPS serve as two non-adaptive baselines. In particular, we consider OPS-Balanced~\citep{wang2018revisiting}, which chooses $\lambda$ to minimize a data-independent upper bound of empirical risk and dominates other OPS variants. 
AdaOPS is one state-of-the-art algorithm for adaptive private regression, which  automatically chooses $\lambda$ by minimizing an upper bound of the data-dependent empirical risk.


We implement OPS-PTR as follows: 
propose a list of $\lambda$ through grid search (we choose $k=30$ and $\lambda$ ranges from $[2.5, 2.5^{10}]$ on a logarithmic scale); instantiate Algorithm~\ref{alg: parameter_ptr} with $\tau =0.1k$, $T=\frac{1}{\tau} \log(1/\delta_2)$ and  $\delta_2 = 1/2 \delta$;
calibrate $\gamma$ to meet the privacy requirement for each $\lambda$. sample $\hat{\theta}$ using $(\lambda,\gamma)$ and return the one with the best validation accuracy. Notice that we use a ``no $\perp$'' variant of Algorithm~\ref{alg:gen_ptr} as the calibration of $\gamma$ is clear given a fixed $\lambda$ and privacy budget (see more details in the appendix). We can propose various combinations of $(\lambda, \gamma)$ for more general applications.


 Figure~\ref{fig:selection}  demonstrates how the MSE error of the linear regression algorithms varies with the privacy budget $\epsilon$. OutPert suffers from the large global sensitivity of output $\theta$. OPS performs well but does not benefit from the data-dependent quantities. AdaOPS is able to adaptively choose $(\lambda, \gamma)$ based on the dataset, but suffers from the estimation error of the data-dependent empirical risk. On the other hand, OPS-PTR selects a  $(\lambda, \gamma)$ pair that minimizes the empirical error on the validation set directly, and the privacy parameter $\gamma$ adapts to the dataset thus achieving the best result.


==> Generalized PTR (1)/relatedwork.tex <==
%\vspace{-1em}
\section{Related Work}
%\vspace{-1em}
\label{sec:related_work}

\textbf{Data-dependent DP algorithms.}
Privately calibrating noise to the local sensitivity is a well-studied problem. One approach is to add noise calibrated to the smooth sensitivity \citep{nissim2007smooth}, an upper bound on the local sensitivity which changes slowly between neighboring datasets. %Smoothed sensitivity considers the local sensitivity of all possible datasets, discounted by their distance to an input dataset $X$.
An alternative to this -- and the focus of our work -- is  Propose-Test-Release (PTR) \citep{dwork2009differential}, which works by calculating the distance $\mathcal{D}_{\beta}(X)$ to the nearest dataset to $X$ whose local sensitivity violates a proposed bound $\beta$. The PTR algorithm then adds noise to $\mathcal{D}_{\beta}(X)$ before testing whether this privately computed distance is sufficiently large.

PTR spin-offs abound. Notable examples include stability-based methods \citep{thakurta2013differentially} (stable local sensitivity of $0$ near the input data) and privately releasing upper bounds of local sensitivity \citep{kasiviswanathan2013analyzing,liu2021differential, decarolis2020end}. We refer readers to Chapter 3 of \citet{vadhan2017complexity} for a concise summary of these classical results. 
Recent work
\citep{wang2022renyi} has provided R\'enyi DP bounds for PTR and demonstrated its applications to robust DP-SGD. Our work (see Section~\ref{subsections:pate}) also considers applications of PTR in data-adaptive private deep learning: Instead of testing the local sensitivity of each gradient step as in \citet{wang2022renyi}, our PTR-based PATE algorithm tests the data-dependent privacy loss as a whole.

\citet{liu2021differential} proposed a new variant called High-dimensional Propose-Test-Release (HPTR). HPTR provides a systematic way of solving DP statistical estimation problems by using the exponential mechanism (EM) with carefully constructed scores based on certain one-dimensional robust statistics, which have stable local sensitivity bounds. HPTR focuses on designing data-adaptive DP mechanisms from scratch; our method, in contrast, converts existing randomized algorithms (including EM and even some that do not satisfy DP) into those with formal DP guarantees. Interestingly, our proposed method also depends on a one-dimensional statistic of direct interest: the data-dependent privacy loss.

 %algorithms.

% The High-dimensional Propose-Test-Release (HPTR) framework \cite{liu2021differential} establishes a unifying characterization of the statistical efficiency of differentially private statistical estimation problems. HPTR releases its output via the exponential mechanism, with a score function whose access to the data depends only on one-dimensional robust statistics (e.g. one-dimensional robust mean or variance). Because these one-dimensional robust statistics have low local sensitivity on resilient\footnote{Resilience of a dataset measures how sensitive the sample statistics are to removing a fraction of the datapoints.} % \footnote{Resilience of a dataset measures how sensitive the sample statistics are to removing a fraction of the datapoints, similar to the finite sample breakdown point of \cite{brunel2020propose}.} 
% datasets, \cite{liu2021differential} can then provide tight local sensitivity bounds and use the PTR mechanism to check that a given dataset satisfies the resilience property.

% Recent work \cite{brunel2020propose} has put forward a more general version of the PTR mechanism for the purpose of deriving concentration inequalities for differentially private median
% and mean estimators. Their algorithm introduces a notion of distance related to the finite sample breakdown point, a measure of statistical robustness which quantifies the smallest fraction of datapoints which can be arbitrarily changed before the estimator diverges. While this allows their PTR algorithm to generalize to a broad class of estimators, the choice of how to inject noise is still restricted to either the Laplace or Gaussian mechanism.



% Our work, in contrast, makes no assumptions about the statistical properties of an input dataset. Instead we focus on developing a flexible framework suitable for any choice of DP mechanism.




\textbf{Data-dependent DP losses.} The flip side of data-dependent DP algorithms is the study of data-dependent DP losses \citep{papernot2018scalable,soria2017individual,wang2017per}, which fix the randomized algorithm but parameterize the resulting privacy loss by the specific input dataset. For example: In the simple mechanism that adds Laplace noise with parameter $b$, data-dependent DP losses are $\epsilon(X) = \Delta_{\text{LS}}(X)/b$. The data-dependent DP losses are often much smaller than the DP loss, but they themselves depend on the data and thus may reveal sensitive information; algorithms satisfying a data-dependent privacy guarantee are not formally DP with guarantees any smaller than that of the worst-case. Existing work has considered privately publishing these data-dependent privacy losses \citep{papernot2018scalable,redberg2021privately}, but notice that privately publishing these losses does not improve the DP parameter of the given algorithm. Part of our contribution is to resolve this conundrum by showing that a simple post-processing step of the privately released upper bound of $\epsilon(\text{Data})$ gives a formal DP algorithm.

% \textbf{On data-dependent DP losses.} In addition to the above, there has been an increasing list of empirical DP work that fix the parameters of a randomized algorithm while reporting the resulting data-dependent DP losses $\epsilon(\text{Data})$ after running on a specific dataset \citep{ligett2017accuracy,papernot2018scalable,zhu2020private, feldman2021individual}. The data-dependent DP losses are often smaller than the worst-case DP losses, but technically speaking, these algorithms are not formally DP with DP guarantees any smaller than that of the worst-case. In addition, the data-dependent DP losses themselves are sensitive, and thus cannot be reported. A typical solution is to privately release $\epsilon(\text{Data})$, but it still does not satisfy DP as this would require a prescribed $(\epsilon,\delta)$-DP parameter to be satisfied for all input datasets. Part of our contribution is to resolve this conundrum by showing that a simple post-processing step of the privately released upper bound of $\epsilon(\text{Data})$ gives a formal DP algorithm.

\textbf{Private hyper-parameter tuning.}
%In addition to normal machine learning parameters (e.g., the learning rate) DP algorithms introduce a few new hyper-parameters, e.g., the clipping threshold in DP-SGD.
Our work has a nice connection with private hyper-parameter tuning. 
%Recent work~\citep{papernot2021hyperparameter} empirically demonstrates that repeat privacy-preserving training and tuning hyper-parameters does leak private information. 
Prior work~\citep{liu2019private, papernot2021hyperparameter} requires each candidate configuration to be released with the same DP (or R\'enyi DP) parameter set. Another hidden assumption is that the parameters must not be privacy-correlated
(i.e., parameter choice will not change the privacy guarantee). Otherwise we need to use the largest DP bound across all candidates.
For example, \citet{liu2019private} show that if each mechanism (instantiated with  one group of hyper-parameters) is $(\epsilon, 0)$-DP, then running a random number of mechanisms and reporting the best option satisfies $(3\epsilon, 0)$-DP. 
Our work directly generalizes the above results by (1) considering a wide range of hyper-parameters, either privacy-correlated or not; and (2) requiring only that individual candidates to have a \emph{testable} data-dependent DP.









==> Generalized PTR (1)/test_construction.tex <==

Classic PTR uses the Laplace mechanism to construct a differentially private upper bound of $\cD_{\beta}(X)$, the distance from input dataset $X$ to the closest dataset whose local sensitivity exceeds the proposed bound $\beta$. The tail bound of the Laplace distribution then ensures that if $\cD_{\beta}(X) = 0$ (i.e. if $\Delta_{LS}(X) > \beta$), then the output will be released with only a small probability $\delta$.

The following theorem shows that we could instead use a differentially private upper bound of the data-dependent DP $\epsilon_{\phi}(X)$ in order to test whether to run the mechanism $\cM_{\phi}$.

\begin{theorem}[Generalized PTR with private upper bound]\label{exp: upperbound}
Suppose we have a differentially private upper bound of $\epsilon_\phi(X)$ w.r.t. $\delta$ such that with probability at least $1-\delta'$, $\epsilon_{\phi }^P(X)>\epsilon_{\phi}(X)$. Further suppose we have an $(\hat{\epsilon}, \hat{\delta})$-DP test $\cT$ such that
\begin{align*}
    T(X) &= \begin{cases}
    1 & \text{ if } \epsilon_{\phi }^P(X) < \epsilon, \\
    0 & \text{ otherwise}.
    \end{cases}
    %\vspace{-1em}
\end{align*}
%\yw{Why do you need it to hold for all $\tilde{\delta}$? I thought we only need $\hat{\delta}$}

Then Algorithm~\ref{alg:gen_ptr} is $(\epsilon +\hat{\epsilon}, \delta +\hat{\delta} + \delta')$-DP. %\vspace{-0.5em}
\end{theorem}

%\vspace{-0.5em}

In Section~\ref{subsections:pate}, we demonstrate that one can upper bound the data-dependent DP through a modification of the smooth sensitivity framework applied on $\epsilon_\phi(X)$. Moreover, in Section~\ref{subsections:private_linear_regression} we provide a direct application of Theorem~\ref{exp: upperbound} with private linear regression by making use of the per-instance DP technique~\citep{wang2017per}.

The applications in Section~\ref{sections:applications} are illustrative of two distinct approaches to constructing the DP test for generalized PTR:

\begin{enumerate}
%\vspace{-0.5em}
    \item Private sufficient statistics release (used in the private linear regression example of Section~\ref{subsections:private_linear_regression}) specifies the data-dependent DP as a function of the dataset and privately releases each data-dependent component. %\vspace{-0.5em}
    \item The second approach (used in the PATE example of Section~\ref{subsections:pate}) uses the smooth sensitivity framework to privately release the data-dependent DP as a whole, and then construct a high-confidence test using the Gaussian mechanism. %\vspace{-0.5em}
    
\end{enumerate}
%\vspace{-0.5em}
These two approaches cover most of the scenarios arising in data-adaptive analysis. For example, in the appendix we demonstrate the merits of generalized PTR in handling data-adaptive private generalized linear models (GLMs)  using private sufficient statistics release. Moreover, sufficient statistics release together with our private hyper-parameter tuning (Algorithm~\ref{alg: parameter_ptr}) can be used to construct data-adaptive extensions of DP-PCA and Sparse-DP-ERM (see details in the future work section).





==> Generalized PTR (1)/unified_framework.tex <==
\section{A Unified Framework}

 In Section~\ref{subsection:reduction} we show how to reduce our generalization to classic PTR.

Why do we want to generalize PTR beyond noise-adding mechanisms? Compared to classic PTR, the generalized PTR framework allows us to be more flexible in both the type of test conducted and also the type of mechanism whose output we wish to release. For many mechanisms, the local sensitivity either does not exist or is only defined for specific data-dependent quantities (e.g., the sensitivity of the score function in the exponential mechanism) rather than the mechanism's output. We give a concrete example in Section~\ref{subsection:private_posterior_sampling}.

In other cases, the local sensitivity exists and can be tested efficiently -- \emph{but} isn't sufficiently descriptive to make full use of data-dependent properties. We give an example in Section~\ref{subsection:report_noisy_max} where considering only the local sensitivity leads to a loose privacy guarantee.
% \blue{private binary voting w/ tighter privacy analysis}
% Moreover, even in the cases of noise-adding mechanisms where PTR seems to be applicable, it does not lead to a tight privacy guarantee. Specifically, by an example of privacy amplification by post-processing (Example~\ref{exp: binary_vote} in the appendix), we demonstrate that the local sensitivity does not capture all sufficient statistics for data-dependent privacy analysis and thus is loose.


Lastly, both classic and generalized PTR could refuse to output anything useful when the test fails. In Section~\ref{subsection:testing_data_DP} we demonstrate how to construct a ``sanitized'' upper bound of the data-dependent DP $\epsilon_\phi(X)$ -- which, unlike local sensitivity, always exists. Furthermore, by deriving this upper bound we can obtain an explicit formula of how to choose the parameter $\phi$ in order to avoid the ``$\perp$'' output.


% \subsection{Reduction to classic PTR}
% \label{subsection:reduction}

% \begin{theorem}[Generalized PTR with distance test]\label{exp: dist_ptr}
% Let $\delta, \delta' > 0$ and define an algorithm $\cA: \cR^d \to \{\perp, \cR^d\}$ as follows.
% Let $\gamma(X)$ denote the distance to the nearest dataset $X''$ such that $\epsilon_{\phi, \hat{\delta}}(X'')>\hat{\epsilon}$, i.e.,
% $\gamma(X) = \min_{X''} \{dist(X, X''):\epsilon_{\phi, \hat{\delta}}(X'')>\hat{\epsilon}\}$. Let $\mathcal{T}$ test whether $ \gamma(X)+ Lap(1/\epsilon)>\frac{\log(1/\tilde{\delta})}{\epsilon}$.
%   $\cA$ returns $\cM_\phi(X)$ if $\mathcal{T}$ passes and otherwise returns $\perp$. Then $\cA$ is $(\epsilon+\hat{\epsilon}, \hat{\delta}+ \tilde{\delta})$-DP. 
% \end{theorem}
% % \blue{Look at this again! Are the deltas correct?}

% % \begin{proof}[Proof sketch]
% % \end{proof}

% Theorem~\ref{exp: dist_ptr} shows that generalized PTR is a \emph{strict} generalization of Propose-Test-Release. For noise-adding mechanisms such as the Laplace mechanism, the sensitivity is proportional to the privacy loss (in both the global and local sense, i.e. $\Delta_{GS} \propto \epsilon$ and $\Delta_{LS} \propto \epsilon(X)$). Therefore for these mechanisms the only difference between privately testing the local sensitivity (Algorithm~\ref{alg:classic_ptr}) and privately testing the data-dependent DP (Theorem~\ref{exp: dist_ptr}) is a change of parameterization.

\subsection{Private posterior sampling}
\label{subsection:private_posterior_sampling}


\begin{example}[Private posterior sampling]\label{exp: posterior}
Let $\cM: \cX\times \cY \to \Theta $ be a private posterior sampling   mechanism~\citep{minami2016differential,wang2015privacy,gopi2022private} for approximately minimizing $F_{X}(\theta)$.

$\cM$ samples $\theta \sim P(\theta)\propto e^{-\gamma(F_X(\theta)+ 0.5\lambda ||\theta||^2)}$ with parameters $\gamma, \lambda$. $\gamma,\lambda$ cannot be appropriately chosen for this mechanism to satisfy DP without going through a sensitivity calculation of $\arg\min F_X(\theta)$. In fact, the global and local sensitivity of the minimizer is unbounded even in linear regression problems, i.e., when $F_X(\theta) = \frac{1}{2}||y-X\theta||^2.$ 
%The local sensitivity $\Delta:=||P_{X,y}(\theta)-P_{X', y'}(\theta)||$ is not well-defined  for the sampling algorithm, thus the standard PTR is not applicable.  

\end{example}
Output perturbation algorithms do work for the above problem when we regularize, but they are known to be suboptimal in theory and in practice \cite{chaudhuri2011differentially}.
% do not achieve the level of utility in theory and in practice when comparing to posterior sampling. 
 



\subsection{Report Noisy-max}
\label{subsection:report_noisy_max}


\subsection{Testing data-dependent DP}
\label{subsection:testing_data_DP}

\begin{comment}
\begin{example}(\emph{Laplace Mechanism}) \label{examp:lap_mech}

Given a function $f: \mathcal{X} \rightarrow \mathbb{R}$, we will define
\begin{align*}
    \mathcal{M}_{\phi}(X) = f(X) + \text{Lap}\left(\phi\right).
\end{align*}
% We'll now derive the data-dependent DP function $\epsilon_{\phi}(X)$ associated with $\mathcal{M}_{\phi}$:
A rote calculation with the Laplace distribution tells us that
\begin{align*}
    \log \dfrac{\text{Pr}[\mathcal{M}_{\phi}(X) = y]}{\text{Pr}[\mathcal{M}_{\phi}(X') = y]} &\leq \dfrac{|f(X) - f(X')|}{\phi}.
\end{align*}
Using the above calculation and  Definition~\ref{def:data_dep_dp},
\begin{align*}
    \epsilon_{\phi}(X) = \max\limits_{X': X' \simeq X} \frac{|f(X) - f(X')|}{\phi} = \frac{\Delta_{LS}(X)}{\phi}.
\end{align*}
We can then verify that choosing $\phi = \beta/\hat{\epsilon}$ and $\hat{\epsilon} = \epsilon$ reduces Algorithm~\ref{alg:no_ls} exactly to Algorithm~\ref{alg:classic_ptr}.
\end{example}
\end{comment}

% Next, we provide another instantiation of generalized PTR through the construction of a high-probability upper bound of $\epsilon_{\phi}(X)$.

% \begin{theorem}[Generalized PTR with private upper bound]\label{exp: upperbound}
% Let $\cT$ first construct a differentially private upper bound of $\epsilon_\phi$ such that with probability at least $1-\tilde{\delta}$, $\epsilon_{\phi, \hat{\delta}}^P(X)>\epsilon_{\phi, \hat{\delta}}(X)$. 
% %\yw{Why do you need it to hold for all $\tilde{\delta}$? I thought we only need $\hat{\delta}$}
% Then $\cT$ %tests whether
% returns ``Pass'' if
% $\epsilon_{\phi, \hat{\delta}}^P(X)< \hat{\epsilon}$, otherwise ``not pass''. 
% %Algorithm $\cA$ returns $\cM_\phi(X)$ if $\cT$ passes else returns $\perp$.  % this is made clear in the alg block already?
% If $\cT$ is $(\epsilon,\delta)$-DP, then  $\cA$ is $(\epsilon +\hat{\epsilon}, \delta +\hat{\delta} + \tilde{\delta})$-DP.
% \end{theorem}
% \blue{Theorem~\ref{exp: upperbound} provides a systematic way of deriving data-dependent DP algorithms by deriving and releasing data-dependent DP losses.}


% In Section~\ref{sec: pate}, we demonstrate that one can upper bound the data-dependent DP through a modification of the smooth sensitivity framework applied on $\epsilon_\phi(X)$. Moreover, we provide a direct application of Example~\ref{exp: upperbound} with private linear regression by making use of the per-instance DP technique~\citep{wang2017per}.



\begin{comment}
Moreover, if $\epsilon_\phi(X)$ admits a global sensitivity $\triangle_\phi$, we can use the tail bound of Laplace distribution for such a construction. \todo{Shall we mention privately release sufficient statistics here?}


\begin{corollary}
Assume that $\epsilon_\phi(X)$ has a global $L_1$ sensitivity $\triangle_\phi$. Let $\cT$ privately test if $\epsilon_{\phi, \hat{\delta}}^P(X) \leq \hat{\epsilon}$, where $\epsilon_{\phi,\hat{\delta}}^P(X):= \epsilon_{\phi, \hat{\delta}}(X)+ \text{Lap}(\frac{\triangle_
\phi}{\epsilon}) + \frac{\triangle_\phi \log(1/\delta)}{\epsilon}$. Then an instantiation of Algorithm~\ref{alg:gen_ptr} with the test $\cT$ satisfies $(\epsilon+\hat{\epsilon}, \delta + \hat{\delta})$-DP.
\end{corollary}
\end{comment}

==> Generalized PTR (1)/which_phi.tex <==
The main limitation of generalized PTR is that one needs to ``propose'' a good guess of parameter $\phi$.  Take the example of $\phi$ being the noise level in a noise-adding mechanism. Choosing too small a $\phi$ will result in a useless output $\perp$, while choosing too large a $\phi$ will add more noise than necessary. Finding this 'Goldilocks' $\phi$ might require trying out many different possibilities -- each of which will consume privacy budget.

% Calculating the data-dependent DP offers a systematic way to find this 'Goldilocks' $\phi$.



==> PTR_calibration.tex <==


%  \vspace{-2mm}
% \subsection{``Which $\phi$ to propose?'' --- Generalized PTR with privacy calibration}
%     \vspace{-2mm}
%The optimism of all data-dependent analyses is to add less noise while maintaining the same or even stronger privacy guarantee compared to its data-independent counterpart. However, PTR approaches require a reasonable guess of the proposed parameter (e.g., $\lambda$ in the linear regression example). Otherwise, it may easily output $\perp$ and be less practical. Noting our generalized PTR takes an extra parameter $\phi$, one may hope to try out various $\phi$ (e.g., different noisy levels in private mean estimation) and return the one with the best utility. 
%In this section,  we propose an improved version of the generalized PTR such that the algorithm takes a list of parameters as input, runs PTR with each of the parameters, and only returns the output with the best utility. We show that the privacy guarantee in $\epsilon$ is independent of the number of $\phi$ that we try.  


% The main limitation of generalized PTR is that one needs to ``propose'' a good guess of parameter $\phi$.  Take the example of $\phi$ being the noise level in a noise-adding mechanism. Choosing too small a $\phi$ will result in a useless output $\perp$, while choosing too large a $\phi$ will add more noise than necessary.

% In this section,  we propose an improved version of generalized PTR such that the algorithm takes a list of parameters as input, runs PTR with each of the parameters, and only returns the output with the best utility. We show that the privacy guarantee in $\epsilon$ is independent of the number of $\phi$ that we try.  

% Formally, let $\phi_1, ..., \phi_k$ be a set of hyper-parameters and $\tilde{\theta}_i \in\{\perp, \text{Range}(\cM)\}$ denotes the output of running generalized PTR on a private dataset $X$ with $\phi_i$. 
% Let $X_{val}$ be a public validation set and $q(\tilde{\theta}_i)$ be the score of evaluating $\tilde{\theta}_i$ with $X_{val}$ (e.g., validation accuracy). The goal is to select a pair of DP model $\tilde{\theta}_i$ and its  hyper-parameter $\phi_i$, such that $\tilde{\theta}_i$ maximizes the validation score.

%(1) the system is $(\tilde{\epsilon}, \tilde{\delta})$-DP; (2) the validation score $q(\theta_i) \geq max_j q(\theta_j) -\alpha$ with high probability.


%The generalized PTR with privacy calibration is described in Algorithm~\ref{alg: parameter_ptr}. Specifically, $T$ denotes the computational limit. We assume an oracle access to the score function $(\tilde{\theta}_i, q(\tilde{\theta}_i)) \sim Q(X)$ by: (a) pick a candidate $\phi_i$ randomly; If there is an order between parameters (e.g., $\phi_i$ denotes the magnitude of noise level), then we can sort $\phi_i$ such that $\phi_1 < \phi_2 < ... < \phi_k$ and pick $\phi_i$ from the left; (b) Run
%Algorithm~\ref{alg:gen_ptr} to obtain $\tilde{\theta}_i$ and evaluate it on $X_{\text{val}}$. Finally, the algorithm outputs the highest scored candidates.


% Finally, the algorithm has a random stopping with probability $\gamma$. 
% state privacy guarantee, cite from 
% The generalized PTR framework with privacy calibration is described in Algorithm~\ref{alg: parameter_ptr}. The privacy guarantee of Algorithm~\ref{alg: parameter_ptr} is an application of \citet{liu2019private}.

% \begin{theorem}[ Theorem 3.4 \citet{liu2019private} ]
% Fix any $\tau \in [0, 1], \delta_2>0$ and let $T =\frac{1}{\tau} \log \frac{1}{\delta_2}$. If each oracle access to $Q(X)$ is $(\epsilon, \delta)$-DP, then
% Algorithm~\ref{alg: parameter_ptr} is $(3\epsilon + 3\sqrt{2\delta}, \sqrt{2\delta} T +\delta_2 )$-DP.%\yw{What if it does not reach $T$? Also in the algorithm it has $k$ right?  Also, did you define which score it is?}
% \end{theorem}
% The theorem implies that one can try a random number of $\phi$ while paying a constant $\epsilon$.
% In practice, we can roughly set $\tau = \frac{1}{10k}$ so that the algorithm is likely to test all $k$ parameters. We emphasize that the privacy and the utility guarantee (see Sec~\ref{sec: omit_gen_ptr} in Appendix) is not our contribution. But the idea of applying a generalized PTR to enforce a uniform DP guarantee over all choices of parameters with data-dependent analysis is new, and in our opinion, significantly broadens the applicability to generic hyperparameter tuning machinery from \citep{liu2019private}.




%\begin{remark}[Private hyper-parameter tuning]
%Our results directly generalize private hyper-parameter tuning. We remark that our PTR-based algorithm can tune privacy parameters (e.g., noise scale) adapted to the data-dependent DP while maximizing the utility. In contrast, prior work~\citep{papernot2021hyperparameter}\citep{liu2019private} on this problem requires a uniform DP guarantee of all base mechanisms, thus not applicable. 
%\end{remark}


%We can categorize hyper-parameters of privacy-preserving models into two sets --- utility parameters and privacy parameters. 

%Most prior work~\citep{liu2019private, papernot2021hyperparameter} on this problem assumes parameters of interests are privacy uncorrelated (e.g., regularizer parameter) and require a uniform DP bound for all of the mechanisms $\cM_i$.  \citet{liu2019private} shows that if each mechanism $\cM_i$ is $(\epsilon, 0)$-DP, then run a random number of mechanisms and report the best option satisfies $(3\epsilon, 0)$-DP.

 %On the other hand, for noise calibration with a fixed privacy budget, we note that one could naively apply a differential privacy accountant (e.g., Renyi DP accountant \citep{mironov2017renyi}) to apriori optimize the privacy parameters with a fixed privacy budget. However, this approach does not give us insights into the utility guarantee or take advantage of the data-dependent property. 

%We generalize the above results by: (1) considering a wide range of hyper-parameters that could be either privacy parameters or non-privacy parameters. (2) Tune parameters adapted to the dataset itself.

%\yw{The two paragraphs above are not clear (from ``on the other hand'' onwards). Should  revise so readers understand what you mean.} % i have remove it to the related work.


% \begin{algorithm}[t]
% 	\caption{PTR with hyper-parameter selection}
% 	\label{alg: parameter_ptr}
% 	\begin{algorithmic}[1]
% 	   \STATE {\textbf{Input}:  Privacy budget $\epsilon, \delta$, cut-off $T$, parameters $\phi_{1:k}$, flipping probability $\tau$ and the access to the validation score $q(\cdot)$. } 
% 		\STATE {Initialize the set $S=\varnothing$.}
% 		\STATE{Draw $G$ from a geometric distribution $\cD_\tau$ and let $\hat{T}=\text{min}(T, G)$.}
% 		\FOR{i = 1 ,..., $\hat{T}$}
% 		\STATE{ pick a random $\phi_i$ from $\phi_{1:k}$.}
% 		\STATE{evaluate $\phi_i$: $(\tilde{\theta}_i, q(\tilde{\theta}_i))\gets$ Algorithm~\ref{alg:gen_ptr}($\phi_i, (\epsilon, \delta)$).}
% 		\STATE {$S \gets S \cup \{\tilde{\theta}_i, q(\tilde{\theta}_i)\}$.}
% 		%\STATE{with probability $\gamma$, we output the highest scored candidate from $S$ and halt.}
% 		\ENDFOR	\vspace{-1mm}
% 	\STATE{Output the highest scored candidate from $S$.}
% 	\end{algorithmic}
% 	\vspace{-1mm}
% \end{algorithm}

% \begin{figure*}[t]
% 	\centering	
% 	\subfigure[Bike dataset]{
% 	\includegraphics[width=0.48\textwidth]{img/bike.pdf}\label{fig:bike}}
% 	\subfigure[Elevators dataset]{
% 	\includegraphics[width=0.48\textwidth]{img/elevator.pdf}\label{fig:ele}}
% 	\vspace{-2mm}
% 	\caption{Differential private linear regression algorithms on UCI datasets. $y$-axis reports the MSE error with confidence intervals. $\epsilon$ is evaluated with $\delta = 1e-6$. }
% 	\label{fig:selection}\vspace{-2mm}
% \end{figure*}

\textbf{Case study with private linear regression.}
We next apply Algorithm~\ref{alg: parameter_ptr} to the private linear regression task with UCI regression datasets. Standard z-scoring is applied and each data point is normalize with a Euclidean norm of 1.  We consider $(60\%,10\%,30\%)$ splits for training, validation and testing test.

\textbf{Baselines}
\begin{itemize}
\vspace{-2mm}
    \item Output Perturbation (Outpert)~\citep{chaudhuri2011differentially}: $\theta=(X^TX + \lambda I)^{-1}X^T\bf{y}$. Release $\hat{\theta} = \theta + \bf{b}$ with an appropriate $\lambda$ and $\bf{b}$ is a Gaussian random vector.\vspace{-2mm}
    \item Posterior sampling (OPS). Sample $\hat{\theta}\sim P(\theta)\propto e^{-\gamma(F(\theta)+ 0.5 \lambda ||\theta||^2)}$ with parameters $\gamma, \lambda$.\vspace{-1.5mm}
    \item Adaptive posterior sampling (AdaOPS)~\citep{wang2018revisiting}. Run OPS with $(\lambda, \gamma)$ chosen adapted to the dataset.\vspace{-1.5mm}
\end{itemize}
%\yw{\cite{gopi2022private} had a nice and clean Gaussian DP bound for OPS. I thought if we can privately test the strong convexity from the dataset, it should satisfy a stronger Gaussian DP. How are privacy accounted in the experiments now?} % use composition.  Each oracle call is (eps, delta). split (epsilon/2, delta/2) to release data dependent quantity, use the remaining to tune gamma for an input lambda.
Outpert and OPS serve as two non-adaptive baselines. In particular, we consider OPS-Balanced~\citep{wang2018revisiting}, which chooses $\lambda$ to minimize a data-independent upper bound of empirical risk and dominates other OPS variants. 
AdaOPS is one state-of-the-art algorithm for adaptive private regression, which  automatically chooses $\lambda$ by minimizing an upper bound of data-dependent empirical risk.


We implement OPS-PTR as follows: 
propose a list of $\lambda$ through grid search (we choose $k=30$ and $\lambda$ ranges from $[2.5, 2.5^{10}]$ on a logarithmic scale); instantiate Algorithm~\ref{alg: parameter_ptr} with $\tau =0.1k, T=\frac{1}{\tau} \log(1/\delta_2)$ and  $\delta_2 = 1/2 \delta$;
calibrate $\gamma$ to meet the privacy requirement for each $\lambda$. sample $\hat{\theta}$ using $(\lambda,\gamma)$ and return the one with the best validation accuracy. Notice that we use a ``no $\perp$'' variant of Algorithm~\ref{alg:gen_ptr} as the calibration of $\gamma$ is clear given a fixed $\lambda$ and privacy budget (see more details in the appendix). We can propose various combinations of $(\lambda, \gamma)$ for more general applications.


 Figure~\ref{fig:selection}  demonstrates how  the MSE error of the linear regression algorithms vary with the privacy budget $\epsilon$. OutPert suffers from the large global sensitivity of output $\theta$. OPS performs well but does not benefit from the data-dependent quantities. Alternatively, AdaOPS is able to choose $(\lambda, \gamma)$ adapted to the dataset, but suffers from the estimation error of the data-dependent empirical risk. On the other hand, OPS-PTR chooses a  $(\lambda, \gamma)$ pair that minimizes the empirical error on the validation set directly, and the privacy parameter $\gamma$ is adapted to the dataset thus achieving the best result.




==> expost.tex <==

\subsection{Ex-post DP}

\begin{theorem}
Algorithm~\ref{alg: ptr_gen_post} is $(\max(\epsilon_1 +\epsilon_2, \epsilon_2 -\epsilon_1 +\nu), 2\delta_2 +e^{\epsilon_2}\cdot \delta)$-DP if with probability at least $1-\delta$, we have $\epsilon(\theta, X)\leq \epsilon_\phi(X, \theta)^p\leq \epsilon_\phi(X,\theta) + \nu$ for any neighboring dataset $X'$.
\end{theorem}

\begin{proof}

Let $\tilde{\cM}$ denote Algorithm~\ref{alg: ptr_gen_post}.
We consider two cases: $\tilde{\cM}(X)=\perp$ and $\tilde{\cM}(X)=\theta$.
The probability of outputting $\perp$ can be written explicitly as follows:
\begin{align*}
&\pr[\tilde{\cM}(X)=\perp] = \pr_{\tilde{\cM}(X)}[\epsilon(\theta, X)^p>\epsilon_1]\\
&= \mathbb{E}_{\theta \sim \cM(X)}\bigg[ \pr_{\cA(X, \theta)}[\epsilon(\theta, X)^p >\epsilon_1|\theta]\bigg]\\
&\leq e^{\epsilon_2} \underbrace{{\mathbb{E}_{\theta \sim \cM(X)}\bigg[ \pr_{\cA(X',\theta)}\bigg[\epsilon(\theta, X')^p >\epsilon_1|\theta\bigg]\bigg]}}_{\text{denoted by} (*) } + \delta_2\\
\end{align*}
The inequality in the last line uses the definition of DP of $\cA(X,\theta)$, which satisfies $(\epsilon_2, \delta_2)$-DP.
Then our goal is to bound $(*)$.  Using the assumption ``w.h.p. $1-\delta$, $\epsilon(\theta, X)\leq \epsilon(X, \theta)^p\leq \epsilon(X,\theta) + \nu$, we have 

\[ (*)\leq \mathbb{E}_{\theta \sim \cM(X)}\bigg[ \pr_{\cA(X',\theta)}\bigg[\epsilon(\theta, X')^p >\epsilon_1
\cap E | \theta \bigg]\bigg] + \delta\]
where $E$ denotes the event of $\epsilon(\theta, X)\leq \epsilon(X, \theta)^p\leq \epsilon(X,\theta) + \nu$.

Note that \[\epsilon(\theta, X')^p \leq \epsilon(\theta, X') +\nu = \log \frac{\pr_{\cM(X')}(\theta)}{\pr_{\cM(X)}(\theta)} + \nu\], which combines with $\epsilon(\theta,X')^p>\epsilon_1$, gives us $\log \frac{\pr_{\cM(X)}(\theta)}{\pr_{\cM(X')}(\theta)} \leq -\epsilon_1 + \nu$. This inequality further implies $\pr_{\cM(X)}(\theta)\leq e^{\nu-\epsilon_1}\cdot \pr_{\cM(X')}(\theta)$.

Substituting the above expression to $(*)$ and we obtain
\begin{align*}
&(*) \leq e^{\nu -\epsilon_1}\cdot \mathbb{E}_{\theta \sim \cM(X')} \bigg[\pr_{\cA(X', \theta)}\bigg[\epsilon(X', \theta)^p >\epsilon \cap E \bigg]\bigg] + \delta\\
&\leq e^{-\epsilon_1 + \nu}\cdot \pr[{\tilde{\cM}(X')=\perp}] + \delta
\end{align*}
Therefore, we have 
\begin{align*}
& \pr[\tilde{\cM}(X)=\perp] \leq e^{\epsilon_2}\bigg(e^{-\epsilon_1 +\nu}\cdot \pr[\tilde{\cM}(X')=\perp ]+\delta\bigg)+ \delta_2\\
&= e^{\epsilon_2 -\epsilon_1 +\nu}\cdot \pr[\tilde{\cM}(X')=\perp] + \delta\cdot \epsilon^{\epsilon_2} +\delta_2
\end{align*}
We next proceed to bound the other case --- $\pr[\tilde{\cM}(X) \in S]$, where $S \subset Range(\cM)$.

 The probability of outputting $S \subset Range(\cM)$ is as follows:
 \begin{align}
 & \pr[\tilde{\cM}(X)\in S)] \\
 &= \underbrace{\mathbb{E}_{\theta \sim \cM(X)}\bigg[ \pr_{\cA(X,\theta)}\bigg[  \epsilon(X, \theta)^p\leq \epsilon_1, E|\theta \bigg]\mathbb{1}(\theta\in S)\bigg]}_{\text{denoted by} (*)} + \\
 & \underbrace{\mathbb{E}_{\theta \sim \cM(X)}\bigg[ \pr_{\cA(X,\theta)}\bigg[  \epsilon(X, \theta)^p\leq \epsilon_1, E^c |\theta\bigg] \mathbb{1}(\theta\in S)\bigg]}_{\text{denoted by} (**)}
\end{align}, where $E$ denotes the event of $\epsilon(\theta, X)\leq \epsilon( \theta,X) +\nu$.
Similarly, we apply the post-processing property on $(*)$ and we have
\begin{align}
&(*)\leq \mathbb{E}_{\theta \sim \cM(X)}\bigg[\bigg( \pr_{\cA(X',\theta)}[\epsilon(\theta, X')\leq \epsilon(\theta, X')^p\leq \epsilon_1|\theta]\cdot \epsilon^{\epsilon_2}+\delta\bigg)
\mathbb{1}(\theta \in S)\bigg]\\
&\leq e^{\epsilon_2}\int_S \pr[\cM(X)=\theta]\pr_{\cA(\theta, X')}[\epsilon(\theta, X')\leq \epsilon(\theta, X')^p \leq \epsilon_1]d\theta + \delta_2\\
&=e^{\epsilon_2}\int_S \int_{\epsilon(\theta, X')}^{\epsilon_1} \pr[\cM(X)=\theta]\pr_{\cA(\theta, X')}[\epsilon(\theta, X')^p]d \epsilon(\theta, X')^p d\theta + \delta \label{ine: change}\\
&\leq e^{\epsilon_2}\int_S \int_{\epsilon(\theta, X')}^{\epsilon_1}e^{\epsilon_1} \pr[\cM(X')=\theta] \pr_{\cA(\theta, X')}
\epsilon(\theta, X')^p d\epsilon(\theta, X')^pd\theta +\delta_2\\
&=e^{\epsilon_1 +\epsilon_2}\mathbb{E}_{\theta\sim \cM(X')}\bigg[ \pr_{\cA(\theta, X')}[\epsilon(\theta,X')\leq \epsilon(\theta, X')^p \leq \epsilon_1|\theta]\cdot \mathbb{1}(\theta \in S)\bigg] + \delta_2\\
&\leq e^{\epsilon_1 + \epsilon_2} \pr_{\theta \sim \cM(X')}[\theta \in S]+\delta_2
\end{align}
In Inequality~\ref{ine: change}, $\epsilon(\theta, X')^p \leq \epsilon_1 $ implies $\pr(\cM(X)=\theta)\leq e^{\epsilon_1}\cdot \pr[\cM(X')=\theta]$, which allows us to replace $\cM(X)=\theta$ with $\cM(X')=\theta$ in the next step.
For $(**)$, given that $\pr_{\cA(\theta, X)}[\epsilon(\theta, X)>\epsilon(\theta,X')^p]\leq \delta$, we have $(**)\leq \delta$. Therefore, we have 
\[\pr[\tilde{\cM}(X)\in S] \leq e^{\epsilon_1 + \epsilon_2 } \pr[\tilde{\cM}(X')\in S] + \delta_2 + \delta
\]
Combine the case of $\tilde{\cM}(X)=\perp$ and $\tilde{\cM}(X)\in \{Range(\cM)\}$, we have $\forall \tilde{S} \subset \{ Range(\cM) \cup \{\perp\}\}$:
\begin{align*}
    &\pr[\tilde{\cM}(X)\in \tilde{S}] = \pr[\tilde{\cM}(X) \in \tilde{S} \cap \perp^c] + \pr[\tilde{\cM}(X) = \perp]\\
    &\leq e^{\epsilon_1 + \epsilon_2}\pr[\tilde{\cM}(X) \in \tilde{S} \cap \perp^c] + e^{\epsilon_2 -\epsilon_1 +\nu}\pr[\tilde{\cM}(X')=\perp] + 2\delta_2 + e^{\epsilon_2} \delta
\end{align*}
\end{proof}

==> unified_framework.tex <==
\section{A Unified Framework}

 In Section~\ref{subsection:reduction} we show how to reduce our generalization to classic PTR.

Why do we want to generalize PTR beyond noise-adding mechanisms? Compared to classic PTR, the generalized PTR framework allows us to be more flexible in both the type of test conducted and also the type of mechanism whose output we wish to release. For many mechanisms, the local sensitivity either does not exist or is only defined for specific data-dependent quantities (e.g., the sensitivity of the score function in the exponential mechanism) rather than the mechanism's output. We give a concrete example in Section~\ref{subsection:private_posterior_sampling}.

In other cases, the local sensitivity exists and can be tested efficiently -- \emph{but} isn't sufficiently descriptive to make full use of data-dependent properties. We give an example in Section~\ref{subsection:report_noisy_max} where considering only the local sensitivity leads to a loose privacy guarantee.
% \blue{private binary voting w/ tighter privacy analysis}
% Moreover, even in the cases of noise-adding mechanisms where PTR seems to be applicable, it does not lead to a tight privacy guarantee. Specifically, by an example of privacy amplification by post-processing (Example~\ref{exp: binary_vote} in the appendix), we demonstrate that the local sensitivity does not capture all sufficient statistics for data-dependent privacy analysis and thus is loose.


Lastly, both classic and generalized PTR could refuse to output anything useful when the test fails. In Section~\ref{subsection:testing_data_DP} we demonstrate how to construct a ``sanitized'' upper bound of the data-dependent DP $\epsilon_\phi(X)$ -- which, unlike local sensitivity, always exists. Furthermore, by deriving this upper bound we can obtain an explicit formula of how to choose the parameter $\phi$ in order to avoid the ``$\perp$'' output.


% \subsection{Reduction to classic PTR}
% \label{subsection:reduction}

% \begin{theorem}[Generalized PTR with distance test]\label{exp: dist_ptr}
% Let $\delta, \delta' > 0$ and define an algorithm $\cA: \cR^d \to \{\perp, \cR^d\}$ as follows.
% Let $\gamma(X)$ denote the distance to the nearest dataset $X''$ such that $\epsilon_{\phi, \hat{\delta}}(X'')>\hat{\epsilon}$, i.e.,
% $\gamma(X) = \min_{X''} \{dist(X, X''):\epsilon_{\phi, \hat{\delta}}(X'')>\hat{\epsilon}\}$. Let $\mathcal{T}$ test whether $ \gamma(X)+ Lap(1/\epsilon)>\frac{\log(1/\tilde{\delta})}{\epsilon}$.
%   $\cA$ returns $\cM_\phi(X)$ if $\mathcal{T}$ passes and otherwise returns $\perp$. Then $\cA$ is $(\epsilon+\hat{\epsilon}, \hat{\delta}+ \tilde{\delta})$-DP. 
% \end{theorem}
% % \blue{Look at this again! Are the deltas correct?}

% % \begin{proof}[Proof sketch]
% % \end{proof}

% Theorem~\ref{exp: dist_ptr} shows that generalized PTR is a \emph{strict} generalization of Propose-Test-Release. For noise-adding mechanisms such as the Laplace mechanism, the sensitivity is proportional to the privacy loss (in both the global and local sense, i.e. $\Delta_{GS} \propto \epsilon$ and $\Delta_{LS} \propto \epsilon(X)$). Therefore for these mechanisms the only difference between privately testing the local sensitivity (Algorithm~\ref{alg:classic_ptr}) and privately testing the data-dependent DP (Theorem~\ref{exp: dist_ptr}) is a change of parameterization.

\subsection{Private posterior sampling}
\label{subsection:private_posterior_sampling}


\begin{example}[Private posterior sampling]\label{exp: posterior}
Let $\cM: \cX\times \cY \to \Theta $ be a private posterior sampling   mechanism~\citep{minami2016differential,wang2015privacy,gopi2022private} for approximately minimizing $F_{X}(\theta)$.

$\cM$ samples $\theta \sim P(\theta)\propto e^{-\gamma(F_X(\theta)+ 0.5\lambda ||\theta||^2)}$ with parameters $\gamma, \lambda$. $\gamma,\lambda$ cannot be appropriately chosen for this mechanism to satisfy DP without going through a sensitivity calculation of $\arg\min F_X(\theta)$. In fact, the global and local sensitivity of the minimizer is unbounded even in linear regression problems, i.e., when $F_X(\theta) = \frac{1}{2}||y-X\theta||^2.$ 
%The local sensitivity $\Delta:=||P_{X,y}(\theta)-P_{X', y'}(\theta)||$ is not well-defined  for the sampling algorithm, thus the standard PTR is not applicable.  

\end{example}
Output perturbation algorithms do work for the above problem when we regularize, but they are known to be suboptimal in theory and in practice \cite{chaudhuri2011differentially}.
% do not achieve the level of utility in theory and in practice when comparing to posterior sampling. 
 



\subsection{Report Noisy-max}
\label{subsection:report_noisy_max}


\subsection{Testing data-dependent DP}
\label{subsection:testing_data_DP}

\begin{comment}
\begin{example}(\emph{Laplace Mechanism}) \label{examp:lap_mech}

Given a function $f: \mathcal{X} \rightarrow \mathbb{R}$, we will define
\begin{align*}
    \mathcal{M}_{\phi}(X) = f(X) + \text{Lap}\left(\phi\right).
\end{align*}
% We'll now derive the data-dependent DP function $\epsilon_{\phi}(X)$ associated with $\mathcal{M}_{\phi}$:
A rote calculation with the Laplace distribution tells us that
\begin{align*}
    \log \dfrac{\text{Pr}[\mathcal{M}_{\phi}(X) = y]}{\text{Pr}[\mathcal{M}_{\phi}(X') = y]} &\leq \dfrac{|f(X) - f(X')|}{\phi}.
\end{align*}
Using the above calculation and  Definition~\ref{def:data_dep_dp},
\begin{align*}
    \epsilon_{\phi}(X) = \max\limits_{X': X' \simeq X} \frac{|f(X) - f(X')|}{\phi} = \frac{\Delta_{LS}(X)}{\phi}.
\end{align*}
We can then verify that choosing $\phi = \beta/\hat{\epsilon}$ and $\hat{\epsilon} = \epsilon$ reduces Algorithm~\ref{alg:no_ls} exactly to Algorithm~\ref{alg:classic_ptr}.
\end{example}
\end{comment}

% Next, we provide another instantiation of generalized PTR through the construction of a high-probability upper bound of $\epsilon_{\phi}(X)$.

% \begin{theorem}[Generalized PTR with private upper bound]\label{exp: upperbound}
% Let $\cT$ first construct a differentially private upper bound of $\epsilon_\phi$ such that with probability at least $1-\tilde{\delta}$, $\epsilon_{\phi, \hat{\delta}}^P(X)>\epsilon_{\phi, \hat{\delta}}(X)$. 
% %\yw{Why do you need it to hold for all $\tilde{\delta}$? I thought we only need $\hat{\delta}$}
% Then $\cT$ %tests whether
% returns ``Pass'' if
% $\epsilon_{\phi, \hat{\delta}}^P(X)< \hat{\epsilon}$, otherwise ``not pass''. 
% %Algorithm $\cA$ returns $\cM_\phi(X)$ if $\cT$ passes else returns $\perp$.  % this is made clear in the alg block already?
% If $\cT$ is $(\epsilon,\delta)$-DP, then  $\cA$ is $(\epsilon +\hat{\epsilon}, \delta +\hat{\delta} + \tilde{\delta})$-DP.
% \end{theorem}
% \blue{Theorem~\ref{exp: upperbound} provides a systematic way of deriving data-dependent DP algorithms by deriving and releasing data-dependent DP losses.}


% In Section~\ref{sec: pate}, we demonstrate that one can upper bound the data-dependent DP through a modification of the smooth sensitivity framework applied on $\epsilon_\phi(X)$. Moreover, we provide a direct application of Example~\ref{exp: upperbound} with private linear regression by making use of the per-instance DP technique~\citep{wang2017per}.



\begin{comment}
Moreover, if $\epsilon_\phi(X)$ admits a global sensitivity $\triangle_\phi$, we can use the tail bound of Laplace distribution for such a construction. \todo{Shall we mention privately release sufficient statistics here?}


\begin{corollary}
Assume that $\epsilon_\phi(X)$ has a global $L_1$ sensitivity $\triangle_\phi$. Let $\cT$ privately test if $\epsilon_{\phi, \hat{\delta}}^P(X) \leq \hat{\epsilon}$, where $\epsilon_{\phi,\hat{\delta}}^P(X):= \epsilon_{\phi, \hat{\delta}}(X)+ \text{Lap}(\frac{\triangle_
\phi}{\epsilon}) + \frac{\triangle_\phi \log(1/\delta)}{\epsilon}$. Then an instantiation of Algorithm~\ref{alg:gen_ptr} with the test $\cT$ satisfies $(\epsilon+\hat{\epsilon}, \delta + \hat{\delta})$-DP.
\end{corollary}
\end{comment}
